Combining Aggregation and Sampling (Nearly) Optimally for Approximate Query Processing

Sample-based approximate query processing (AQP) suffers from many pitfalls such as the inability to answer very selective queries and unreliable confidence intervals when sample sizes are small. Recent research presented an intriguing solution of combining materialized, pre-computed aggregates with sampling for accurate and more reliable AQP. We explore this solution in detail in this work and propose an AQP physical design called PASS, or Precomputation-Assisted Stratified Sampling. PASS builds a tree of partial aggregates that cover different partitions of the dataset. The leaf nodes of this tree form the strata for stratified samples. Aggregate queries whose predicates align with the partitions (or unions of partitions) are exactly answered with a depth-first search, and any partial overlaps are approximated with the stratified samples. We propose an algorithm for optimally partitioning the data into such a data structure with various practical approximation techniques.

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}

==> coverletter.tex <==
\begin{center}
\textbf{Cover Letter}    
\end{center}
We thank the reviewers for their careful review of our submission and have addressed every point laid out in the reviews. 

\vspace{0.5em} \noindent \emph{Summary of our submission. } We contributed a new synopsis data structure for Approximate Aggregate Query Processing. Precomputation-Assisted Stratified Sampling (PASS) builds a tree of partial aggregates that cover different partitions of a dataset, and associated with the leaf nodes are samples of those partitions. We present a framework for optimally constructing such a data structure and practical algorithms that come close to this optimum. 

\vspace{0.5em} \noindent \emph{Summary of our revision. } The reviewers requested several new experiments and comparisons to recent AQP systems: VerdictDB~\cite{park2018verdictdb}, DeepDB~\cite{hilprecht2019deepdb}, and Result-Reuse~\cite{galakatos2017revisiting}. We found that PASS compares favorably to these frameworks in terms of query latency, space, and result accuracy. Results for VerdictDB and DeepDB are included in the paper (Section \ref{sec:otherbaselines}), and results for baseline inspired by Galakatos et al.~\cite{galakatos2017revisiting} are included in the cover letter (Section \ref{sec:revistreuse}). These experiments were an insightful suggestion by the reviewers, because counter-intuitively, synopsis size is not perfectly correlated with query latency, e.g., systems like VerdictDB require far more memory than PASS but have similar query latencies.  We add new discussion and experiments to Section \ref{sec:endtoend} showing that PASS can control for both space and latency, and the effects of those knobs on result accuracy. Additionally, the reviewers had several concerns about copy editing and clarity. We have thoroughly copy-editted the manuscript fixing all grammatical errors, and notation inconsistencies. 

\vspace{1.0em} \noindent \emph{}

Below are the detailed changes in response to the issues raised by each reviewer. We have highlighted revisions to the text requested by reviewer 1 using a red text color, reviewer 2 using blue, reviewer 3 using green, and for multiple reviewers/changes not explicitly requested by the reviewers with purple.

\vspace{.5cm}
\noindent{\textbf{Reviewer \#1}}

\Rev{R1.O1}{Can you give more evidence on the extensive usage of aggregate queries; for example, 10\% of the database queries are aggregate queries, and they are used frequently every day etc.?}

\Ans{We added the following reference to the introduction: Agarwal et al. studied production SQL workload traces at Facebook (~69k queries)~\cite{agarwal2013blinkdb_}. Roughly 30\% of this workload consists of aggregate queries over tables larger than 1TB, which is ideal for approximate query processing applications. Furthermore, the predicates of these aggregate queries are highly concentrated over a small number of columns: only 211 unique query column sets (sets of columns touched by a query predicate) span more than 68k of the queries in the Facebook trace.}

\Rev{R1.O2}{PASS only supports SUM/COUNT/AVG queries. It is not extendable for other query types (because of the nature of the data structure and the complexity of optimization for large query space).}

\Ans{We clarify that PASS supports MIN, MAX, SUM, COUNT, and AVG queries in Section \ref{sec:ds_and_query_processing}. This is no more restrictive than related work on approximate query processing; for example, AQP++ only supports SUM, COUNT, and AVG queries.}

\Rev{R1.O3}{In Algorithm 1, I think it is necessary to add an if statement at the beginning of the algorithm to check this:

IF intersection(Pi, q(P)) == {} :
RETURN {}

Now the algorithm returns all the leaves, even those in Rnone, creating a non-minimal set.
In the end, the algorithm returns C, which is not defined inside the algorithm.}

\Ans{Thanks! Fixed.}


\Rev{R1.O4}{ There are some user-defined input parameters (e.g., sample size, precomputation cost, ...) that strongly affect the performance and accuracy of the algorithm, and it is not mentioned that how these parameters are chosen. Moreover, the parameters may be hard to tune for regular users.
}

\Ans{Section \ref{tuning} clarifies how we tune the parameters. We summarize below:

\begin{enumerate}
    \item \textbf{Sample Size} The sample size is directly correlated to query latency and storage. We envision that the user gives us either a latency constraint (as described in the paper) or a storage constraint, and the system would translate this into a maximum possible sample size. \emph{Our contributed optimization algorithm will find a PASS structure that optimizes query accuracy under this constraint.}
    \item \textbf{Number of leaf nodes $k$.}  The number of leaf nodes $k$ is proportional to the precomputation cost, and in a balanced tree, setting $k$ defines the entire tree structure. We've now significantly simplified the discussion in Section 4.3.1 to make this clear. Our algorithm for constructing the partition tree has precomputation time of $O(k\cdot m \cdot \log m)$, where $m$ is the number of samples and $k$ the number of partitions. $k$ similarly controls the maintenance time of the data structure (number of nodes to update), and time to reoptimize the structure.
\end{enumerate}

Of the two, the $k$ parameter is a bit more opaque, but we have found that optimization algorithm is quite forgiving and that accuracy is not all that sensitive to the particular choice of parameters.  
Table \ref{tbl:cost} shows the preprocessing cost in seconds required by PASS given different number of partitions ($k$ in the table) on the NYC Taxi dataset. We use a fixed sample rate of 0.0025\%. As expected, the precomputation cost increases as we increase $k$. The results suggest that as we increases $k$, the latency decreases and the accuracy increases, this is because a fine grained partitioning can lead to a more aggressive data skipping and a more efficient sampling.

% This table is to be replaced by PASS-Faster. using smaller sample rates.
% \begin{table}[ht]
% \begin{tabular}{ccccc}
% $k$ & Cost (s) & Avg Latency (s) & Max Latency (s) & Median RE \\ \hline
% 4 & 177 & 0.161788 & 0.590554 & 0.76\% \\ \hline
% 8 & 179 & 0.0852749 & 0.285030 & 0.37\% \\ \hline
% 16 & 181 & 0.0608087 & 0.254699 & 0.22\% \\ \hline
% 32 & 185 & 0.033974 & 0.074441 & 0.11\% \\ \hline
% 64 & 190 & 0.0276496 & 0.095684 & 0.05\% \\ \hline
% 128 & 200 & 0.0231217 & 0.042326 & 0.02\% \\ \hline
% \end{tabular}
% \caption{Preprocessing cost, latency and accuracy given different number of partitions.}
% \label{tbl:cost}
% \end{table}

%This table is to be replaced by PASS-Faster. i.e. using smaller sample rates.
%The accuracy and are very close to prev results, so I only update the cost(s)
%latency are the same.
%W/ 20x-PASS (approximate the online version)
% for 128 we set min_sample_per_bucket to 2 to work with 0.000025 (i.e. more samples, more costs)
% record partitioning time + tree construction time.
\begin{table}[ht]
\begin{tabular}{|c|c|c|c|c|}
\hline
$k$ & Construction Cost(s) & Avg. Latency(ms) & MaxLatency(ms) & MedianRE \\ \hline
4 & 16 & 14.6 & 29.2 & 0.55\% \\  %10+6
8 & 18 & 13 & 26 & 0.32\% \\  %10+8
16 & 20 & 11.6 & 23.3 & 0.18\% \\  %10+10
32 & 22 & 10.7 & 21.4 & 0.11\% \\  %10+12
64 & 25 & 8.9 & 17.8 & 0.04\% \\  %10+15, in table 1 the cost was averaged over 3 datasets. here it is only for NYC dataset.
128 & 50 & 6.4 & 12.9 & 0.03\% \\ \hline %32+18
\end{tabular}
\caption{Preprocessing cost, mean latency, max latency and accuracy given different number of partitions.}
\label{tbl:cost}
\end{table}

Unfortunately, due to limited space, we will exclude this experiment from the paper (but will include the results in an extended version if accepted).}

\Rev{R1.O5}{They mentioned three Hybrid AQPs: Galactos et al. and SampleClean and AQP++, and they only compared their algorithm with AQP++;.
}
\Ans{While similar in spirit, the problem settings and assumptions in above-mentioned work are slightly different and hard to directly compare system-to-system. SampleClean [37] focuses on estimation from samples that have been transformed by data cleaning operations so it is not directly applicable. Galakatos et al. \cite{galakatos2017revisiting} focus on opportunistic reuse of results from previously issued queries without paying expensive preprocessing costs. 

Instead, we ran an experiment comparing the algorithmic technique used in \cite{galakatos2017revisiting} to re-use previously computed results. This estimate is not sampling-based (as in AQP++ and PASS), and extrapolates based on predicate coverage. Not surprisingly, we find that PASS is a far more effective result estimation technique (Section \ref{sec:revistreuse}). However, it is worth noting that the problem setting and assumed costs are very different.}.


\Rev{R1.O6}{In 4.3, they said: “ Where A[i,j] is optimal solution among the first “i” data items with at most j partitions.” (they also have a grammar mistake here and should add "the" behind optimal.)
What do they mean by first “i” data items? They are using intervals (e.g., form i1 to i2) on this data and calculating variance. I think the data item’s order is affecting their calculations, which should not.
}
\Ans{We apologize for the confusing terminology. We first sort the samples (with respect to their predicate values) and we run a dynamic programming algorithm over the sorted samples--leading to a consistent ordering of tuples. We made it clear in the text now.}

\Rev{R1.O7}{The authors did a great job of reducing Median Relative Error, for example, from 0.008 to 0.006 in some cases but with a significant upfront cost. They didn’t mention how much accuracy is needed in real-life queries( or some examples that show state-of-the-art accuracies are not enough). Is it beneficial to occupy space and spend time building a data structure for small improvements ( sometimes)?
}

\Ans{To answer this question, we additionally compared PASS with two state-of-the-art AQP baselines: VerdictDB, DeepDB. These are recently published AQP systems, and we compared performance on all axes: construction cost, storage, query latency, and accuracy. 
Table \ref{tab:full-benchmark-verdict-deep} shows that PASS \emph{has a higher accuracy than these systems while roughly controlling for all of these other axes}. In the (admittedly) narrow setting of ``single table'' approximate query processing, we find that PASS meets all of the performance constraints of recently published systems while achieving higher accuracy. 

With appropriate engineering, we believe that the performance of PASS could be even better. We are particularly encouraged by how storage-efficient PASS is compared to alternatives. We have identified network packet analysis on embedded hardware as a potential application where PASS could apply while more expensive frameworks (like VerdictDB, DeepDB) could not. }

\Rev{R1.O8}{English problems (typos/ grammar).}
\Ans{Fixed!}

\vspace{.5cm}
\noindent{\textbf{Reviewer \#2}}

\Rev{R2.O1}{ The lower-level technical details are not always easy to follow, partially because the notation is inconsistent throughout the paper and partly due to a variety of typos (see details below).
}
\Ans{We fixed the typos and the notations so they are consistent now.
}

\Rev{R2.O2}{The paper is missing a discussion about the incremental maintenance costs for the data structure.
}
\Ans{We added a discussion in the end of Section~\ref{sec:OptPart} about the incremental maintenance costs of the data structure. Simply put, PASS can easily handle new insertions while maintaining the statistical consistency of the estimates. However, if there are enough updates to the structure, re-optimization of the partitioning may be needed. We will expand the discussion on the former, but we believe that the latter is out of scope for this current paper and we leave it as a future work.
}

\Rev{R2.O3}{Even if the authors do not do a thorough comparison of their technique with ML-based approaches, I would feel more confident in the relative efficacy of their approach if they could show at least one example where they perform better than an ML-based method such as in ref [38].}

\Ans{Done! This was a great suggestion. In Subsection \ref{sec:otherbaselines}, we add discussion and experiments to compare an ML-based baseline called DeepDB\cite{hilprecht2019deepdb}.}


1. Intro, par 1: “up-to” -> “up to”

\Ans{Fixed}

2. Figure 1: In the 3rd line of the “Answer:”, change 14 to 4

\Ans{Fixed}

3. Intro, par 3: you refer to ref 30 (VerdictDB as an example of using machine learning for query result estimation, but VerdictDB does not use machine learning, Also, in par. 4, “system have” - > “systems have”

\Ans{Fixed}

4. Figure 2: Upper gray table columns are “A” and “V”, but in the leaf nodes below the columns are “A” and “B”.

\Ans{Fixed}

5. p. 2, par. 1: “an partitioning” -> “a partitioning”

\Ans{Done}

6. Presumably, if you want to handle VAR queries, you could also stores sums of squared a-values.

\Ans{Yes! We are confident that we can handle population variance queries in the same way that AVG queries are processed. However, we do suspect they will generally be more inaccurate than the SUM/COUNT/AVG queries presented in the paper due to their higher sensitivity to outliers. }

\vspace{.3cm}

7. p. 2, top of 2nd col: “workload, is more expensive” -> “workload and is”

\Ans{Done}


8. Section 2, par. 3: The “more precise” problem statement does not say anything about accuracy”

\Ans{Done}

9. Sec. 2.1, par. 1: f(.) should be “a function representing any of the supported aggregates”. Also, the third bullet does not make sense. You just want Predicate(t), and not Predicate(a).

\Ans{Done}

10. p. 3: The three bullets below equation (1) should involve Predicate(t), not Predicate (c).

\Ans{Done}

11. p. 3, col. 2: “total number to” -> “total number of”

\Ans{Done}

12. p. 4: I believe that you can tighten both ub and lb. For ub, replace $MAX(R_{partial})$ with the quantity X defined as follows. Let $P_i*$ be the partition in $R_{partial}$ with the highest maximum value, denoted $M_i*$, and let $n_i*$ be the number of points in $P_i*$. Let $m_0$ be the mean over all of the points corresponding to $R_{cover}$ and $n_0$ be the number of these points. Then $X = (m_0 x n_0 + M_i* x n_i*)/ (n_0 + n_i*)$. This corresponds to the assumption that all points in $P_i*$ are equal to $M_i*$, all of them fall in the query range, no points in any of the other partitions in $R_{partial}$ intersect the query. (This also assumes that all points are positive as mentioned in the paper). You can do something similar with lb.

\Ans{While this method might return a correct upper bound in some cases this is not always the case. Assume the following scenario: Let $m_0=1$, $n_0=10$, $M_i^*=5$ and $n_i^*=2$. Then we have that $X=(1*10+5*2)/12 \approx 1.66$. Now, assume that the query contains $10$ more points from another partition in $R_{partial}$ and all of them have values $4<5$. Then the new average is $(10+10+40)/(10+2+10)\approx 2.72>X$. The problem is that the average $m_0$ (of $R_{cover}$) might be very small comparing to the values in $R_{partial}$ so adding more values might increase the average.}


13. p. 4, col 2: The phrase “avoid loading as many samples as possible” is unclear. Also, is PS3 the framework from [34]? Also “used an” -> “used as an”, “summarizes” -> “summaries”, “use Maximum Likelihood Estimates” -> “uses Maximum Likelihood Estimates”

\Ans{Fixed}

14. p. 5, col 2: Maybe change q(P) to P(q) since you are talking about a set of points.

\Ans{Done}

15. Line 10 of Algorithm 1 should be “Return gamma” not “Return C”

\Ans{Done}

16. 2nd par below Algorithm 1: Exactly how do you evaluate the base case in your system? Do you have to do some sort of lexical analysis of the partitioning condition and the query predicates? Do you actually use Algorithm 1 in the special case of 1D data and use the k-d tree otherwise? Also, “test this case each” -> “test each”, “facilitates us” -> “facilitates”


\Ans{Algorithm 1 is used for any dimension $d$. However, the construction of the partition tree is different between $d=1$ and $d>1$. When $d>1$ it is true that the partition tree is actually the k-d tree we constructed.
The base case (line 2) has two conditions: if $P_i\subseteq P(q)$ or $P_i$ is a leaf. We can easily check if $P_i$ is leaf by checking if the current node has any children. For $P_i\subseteq P(q)$, notice that $P_i$ is associated with a partitioning condition which is an interval for $d=1$ or a rectangle for $d>1$. Similarly, the query $q$ is given to our system with a query predicate which is also an interval for $d=1$ or a rectangle for $d>1$. Hence, we can check the condition $P_i\subseteq P(q)$ implicitly, by checking if the query interval (rectangle) fully contains the interval (rectangle) associated with the node. This check takes $O(d)=O(1)$ time. Finally, we fixed the typos!
}

17. Sec. 3.3: what does “if the query is correlated with the data in the partition” mean?

\Ans{Thanks for the close reading. Here, we wanted to emphasize that a query might partially overlap some partitions so we want to apply sampling. We removed this part of the sentence, since this is exactly the definition of a "partial coverage".}


18. Sec. 3.4: In the “partial aggregation” paragraph, you use the terminology “agg” and “part”. You should choose one of these and be consistent. Also, in the definition of agg, I think $N_R/N$ should be replaced by $N_i / N_q$ for the samp + agg addition to work. Note here that “R” has never been defined.

\Ans{Fixed}

19. The notation is inconsistent from Section 3 to Section 4. E.g., in the first displayed equation in Sec. 3.4 you have $w_i^2 V_i(q)$, whereas in the first displayed equation in Section 4.1, you have $w_R^2 V_R(q)$, and I think that both these expressions are supposed to mean the same thing. In the latter equation, R is being used to represent a partition, but previously the variable R always represented a set of partitions.

\Ans{We made the notation consistent between section 3 and 4. Now the error function at Section 4 is defined with the same notation as in Section 3 (we use the new notation $\bucket_i$ to denote the leaf or equivalently the partition $i$ in section 4). Furthermore, we make sure $R$ is always used as the current partitioning, i.e., set of partitions.}

20. Sec. 4.1: How exactly does the number of leaves govern the construction time. Is there a complexity formula? Also, “each leaf will define a” -> “each leaf will define”, and change “rectangular regions” to “rectangular region”.

\Ans{
The construction time of our algorithm is roughly $O(kN \log N)$, (or $O(km \log m)$ where $m$ is the number of samples we use), so we choose $k$ to be the maximum value such that $km\log m\leq \tau_c$. We also fixed the typos.}

21. Section 4.2: You should remind the reader of what $c_i$ is, since it appeared much earlier. Also, why is the complexity $O(N^2)$? If you are segmenting N sequential points into k nonempty partitions to form the leaf nodes, you can this in [(N-1) choose (k-1)] ways.

\Ans{Fixed! It is true that all possible partitions are [(N-1) choose (k-1)]. What we actually mean is that in 1D there are $O(N^2)$ possible queries. So someone could precompute and store the result of all possible queries using $O(N^2)$ space. Ideally, we want to avoid that due to the quadratic dependency on space (and the quadratic precomputation time). We modified the text to make it clear.}

22. It would be nice to provide a sentence or two about the intuition behind Lemma 4 (looking at worst case, etc.)

\Ans{Done}


23. Sec. 4.3: in line (2)(a) of the 1D algorithm, you need g <= C <= w

\Ans{Fixed}

24. Sec. 4.3, par 3: should sqrt(2) be sqrt(k) per Lemma 4.1? also, reformat the equation at the bottom of the page.

\Ans{In lemma 4.1 we show the worst case result. In particular, the approximation factor in lemma 4.1 is sqrt(max number of partially intersected partitions). In the worst case, in higher dimensions, max number of partially intersected partitions is k and that is why we get sqrt(k). However, in 1D the query is an interval and it can only partially intersect at most 2 partitions. This is why we get sqrt(2) in Section 4.3. We added some text to make it more clear.}

25. Sec. 4.4: I don’t understand the last line about the “faster discretization method”

\Ans{Here, we mean that that in higher dimensions we can use the faster discretization method we used in 4.3.1 in 1D.
When we construct the k-d tree we need to have a procedure to decide which leaf node contains the query with the largest variance. A naive way is to consider all possible queries in every leaf. Using the same ideas as in the faster discretization method in 1D (modified for any dimension) we can get a much faster procedure to find the a query with approximately the maximum variance. Due to space limit we do not describe this method in the main text.
We added some text to make it clear.
}

26. Sec. 5.1: How many records in the Taxi dataset?

\Ans{The Taxi dataset contains 7.7 million records. We added it in the text.}

27. 5.1.3: using “R” to denote the budget is probably overloading the notation “R”

\Ans{We changed the notation $R$ from section 5.1.3. Currently, we only use $R$ for a set of partitions.}

28. 5.2.3: “scramble have” -> “scramble has”

\Ans{Done}

29. Sec. 5.4: “expands the node with the smallest depth and breaks ties…then constructs”

\Ans{Done}

30. Sec. 6: “formalize” -> “formalizes”

\Ans{Done}

31. Ref [20]: “olap” -> “OLAP”

\Ans{Done}

\vspace{.5cm}
\noindent{\textbf{Reviewer \#3}}

\Rev{R3.O1}{As their method is both based on sampling and data skipping/aggregate reuse (you are skipping reading the samples from the nodes covered by the aggregate), I feel like the paper would be strong to show their method without sampling the leaf nodes and instead issuing the full query on that partition of data (i.e., a 100\% sample). This could act like a comparison to other data skipping methods (e.g. QuickR) without significant extra work.}

\Ans{This is an intriguing point and we explored in our revision. Data skipping frameworks skip partitions of data that are not relevant to a query. On the other hand, PASS additionally skips partitions that are completely covered by the query. Experiments in Section \ref{sec:dataskipping} illustrate this point. Unfortunately, due to a lack of space (and a prioritization of experiments comparing PASS against VerdictDB and DeepDB), we only include a textual discussion of this point in Section \ref{sec:part}. }


\Rev{R3.O2}{One of the limiting factors of their method seems to be the query set. They support aggregates over one column over a set of predicate columns. How would you do group bys or multiple predicates? I imagine multiple predicates would be multiple trees. What about group bys? A discussion of how'd you do this would greatly strengthen the argument. Further, mining some simple statistics about how covering you query template is (for e.g., over the IDE Bench data) would also help motivate these templates.
}
\Ans{
We added a paragraph ``Extensions'' in the end of Section 4 where we briefly explain how to handle multiple predicates, categorical variables, and group-by.
}

- Fig 3: can you make this larger. It's hard to read with this font.

\Ans{We removed Fig 3 due to page limit.}

\vspace{.3cm}

- Relation work: can you talk about VerdictDB, too. You use that method in the evaluation section but don't talk about that work in the related work. Also, as you say the AQP++ work is the most similar to yours, can you explain that system in a little more detail. E.g. what is the improved optimization algorithm?

\Ans{Done. We have expanded the related work section accordingly.}

- Sec 3.2: Can you give an example of partitions where no such deterministic condition exists.

\Ans{Thanks for the close reading, and have removed this statement since it was confusing.}

%\vspace{.3cm}

- Sec 3.2: what is M? Also, can you explain the intuition behind the $\gamma \log B$ more The "overlaps withs leafs" is a little confusing to me.

\Ans{$M$ is a typo, we changed it to $B$, the number of partitions (strata) we have. Each node of the tree is associated with an interval in $1$D or a rectangle in $d$-dimensions. When we say that a query overlaps with a leaf we mean that the query rectangle intersects the leaf's rectangle. There are three cases: A query rectangle fully contains, partially intersects or does not intersect leaf's rectangle. In the worst case if there are $\gamma$ leaves that partially intersect the query then in each level of the partition tree we might visit $O(\gamma)$ nodes. Hence, if the partition tree is balanced the time query complexity is $O(\gamma \log B)$. We slightly changed the text to make it clear.}

- Sec 4.1: How do you bound the number of nodes and number of samples give limits $\tau_c$ and $\tau_q?$ Is there an equation you use?

\Ans{The construction time of our algorithm is roughly $O(kN \log N)$, (or $O(km \log m)$ where $m$ is the number of samples we use), so we choose $k$ to be the maximum value such that $km\log m\leq \tau_c$. The query time of our data structure in 1D is $O(\log k + m_P)$, where $m_P$ is the number of samples in a partition. Hence, given $\tau_q$ we can decide the number of partitions or we can guarantee an upper bound on the number of samples in each partition.}

- Sec 4.2: Can you discuss a little about the consequences, if any, of the assumption introduced in 4.2.1 about the number of samples being sufficiently large for a partition. In sparse data domains, I'd imagine this may not be true?

\Ans{PASS can answer any query even if this assumption does not hold. However, this is an assumption we make to have theoretical guarantees. We note that it is a reasonable assumption because if a query partially intersects a partition $P_i$ and the query contains less than $\delta m$ samples in $P_i$ then the number of samples is so small that we cannot have a good estimation of the variance of the query in $P_i$. Similarly, if a user asks an extremely selective query (that contains a very small number of samples) PASS (and most AQP systems) will return an answer but it is not clear if the result is a good estimator of the ground truth.}


Evaluation:

- How do you randomly select queries?

\Ans{We generate a query by randomly selecting two values from each attribute domain to form a predicate. Thus, the workload is a uniform distribution over interals.}

- Can you discuss any scalability challenges to handling 1000 of columns with potentially hundreds of columns. No experiments needed, but a brief understanding of the upper limits would be nice. This can be in the conclusion, too.

\Ans{If there are 100 ``aggregation'' columns, we have to construct separate 100 trees, so the primary scaling challenge is in terms of storage space. As our recent experiments show, PASS is highly storage-efficient compared to recently proposed AQP systems~(Table \ref{tab:full-benchmark-verdict-deep}). We are fully confident that PASS can scale to any dataset currently used in AQP.

A more interesting question is to consider how PASS might work if the complexity of the predicates significantly increases (which is not really tested in recent AQP work).  The complexity of constructing a k-d tree partition with theoretical guarantees (using our new faster algorithm) for constant dimension $d$, is $O(n\log^{d-1} n+k\log^{d} n)$ or $O(n+kn^{1-1/d})$ for SUM queries, and  $O(kn\log^{d} n)$ for AVG queries. We added a few sentences in the conclusion as the reviewer suggested.}

- Would it be possible to compare against the Revisiting Reuse paper? Also, why is VerdictDB just in a separate table. Can you not compare it in the other plots?

\Ans{Done! This was a great suggestion. In Subsection \ref{sec:otherbaselines}, we add discussion and experiments to compare PASS with VerdictDB, DeepDB. Comparison with a simplified Revisiting Reuse baseline can be found in Subsection \ref{sec:revistreuse}}.

\begin{appendices}
 \appendix
\section{Appendix}
\subsection{Comparison with Some More Baselines}
As requested and due to page limit, experiments that compare PASS with a data skipping baseline and a Revisiting Reuse baseline can be found below.

\subsubsection{Comparison with a Data Skipping Baseline}
\label{sec:dataskipping}
\onethree{To further demonstrate how PASS would compare with other baselines that enables data skipping without combining sampling, we build a baseline called AGGR. AGGR use the same partitions constructed by PASS, when solving a query, it skips irrelevant partitions and only use the partitions that are intersecting with the query to construct the final answer. More specifically, in this implementation, the answer is given by simply aggregating the summaries of all relevant partitions which leads to a hard upper bound of the ground truth. In practice, we can utilize more sophisticated techniques to decide how the summaries in the partitions can be used to produce the final answer, for example, a weighted sum, etc.}

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\linewidth]{exp-figures/LPA-RESR.pdf}
  \caption{We compare PASS with a baseline that only use aggregates, to demonstrate how PASS performs relative to baselines that utilize data skipping without sampling.}
  \label{fig:lpa-resr}
\end{figure}
\onethree{Results in left plot of Figure \ref{fig:lpa-resr} suggest that the accuracy of both approaches increases as we increase the number of partitions, this is expected because fine grain partitioning make it possible for the approaches to skip more irrelevant partitions to achieve a better result. We also compare the average skip rate of the two approaches, which is the ratio between the number of partitions that are skipped and the total number of partitions. In PASS, by combining sampling with precomputed aggregates, not only we can skip the irrelevant partitions like AGGR does, we can also skip the partitions that are completely covered by the query and only focus on the partitions that are partially intersect with the query.  The right plot of Figure \ref{fig:lpa-resr} shows that the skip rate of AGGR plateaus around 65\% while the skip rate of PASS keep increasing which is expected, for example, in 1D queries, the number of relevant partitions increases with the total number of partitions, but the number of partially intersected partitions is at most 2.}

\subsubsection{Comparison with Revisiting Reuse}
\label{sec:revistreuse}
\onethree{We believe the PASS differs from Revisiting Reuse (RR) \cite{galakatos2017revisiting} in at least two important aspects: 1) RR is designed to be used in a conversational data exploration process in which it can use previous queries to answer future queries, PASS does not limit itself to such a session-like scenario; 2) RR does not require any prior knowledge nor pre-processing. For above reason, the authors of \cite{galakatos2017revisiting} also believe comparing with approaches like VerdictDB which requires pre-processing is not fair and they didn't conduct any experiment in their paper. }

\onethree{Nonetheless, we implement a simplified baseline that captures the main idea of Revisiting Reuse: the baseline make use of the same partition that is created by PASS; it assumes the data is distributed uniformly thus the queries are answered by taking a weighted sum of the intersecting pre-aggregates with the query. The results can be found in \ref{fig:lparr-k}, we can see that on the three real-life dataset, as we vary the number of partitions, the accuracy of both approaches improve and PASS outperforms the simplified Revisiting Reuse baseline.}

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\linewidth]{exp-figures/LPARR-RE-k.pdf}
  \caption{On the three real-life datasets, we compare PASS with a simplified Revisiting Reuse baseline that use the same aggregates generated by PASS to answer query given an assumption of uniform data distribution.}
  \label{fig:lparr-k}
\end{figure}


\end{appendices} 

==> design.tex <==

\section{Design}
For communication purpose and to exclude from the paper later, you can find the UML in Figure \ref{fig:uml} and the structure diagram in Figure \ref{fig:sampletree}.

\subsection{A Qualitative Analysis of the Design}

To understand how different components of our design benefit query execution, we compare our baseline with AQP++ qualitatively.

Let's assume our PA tree contains $h$ layers with a leaf layer that contains a partition $P_h$. Let the fan-out factor be $\zeta$, we have $|P_{h-1}| = |P_h|/\zeta$. The AQP++ baseline use the same partition $P_h$. Our baseline VAST is a hybrid of the PA tree and stratified sampling. 

We consider three typical queries:

Q1: contains a predicate that perfectly aligns with the partition $P_h$, i.e. the query can be solved perfectly without using sampling by AQP++.

Q2: contains a predicate that introduce an redundant area of size $\Delta_h$ when map to $P_h$, and $\Delta_{h-1} = \Delta_{h}$, i.e. increasing the partition granularity from $P_{h-1}$ to $P_{h}$ does not decrease the redundant area.

Q3: contains a predicate that introduce an redundant area of size $\Delta_h$ when map to $P_h$, and $\Delta_{h-1} > \Delta_{h}$, i.e. increasing the partition granularity decrease the redundant area.

Now assume we want to solve each of the queries to achieve an target accuracy of $\alpha_t$, we compare the cost of the two baselines, we measure two costs: 1) the cost of using PA-nodes, i.e., the number of PA-nodes used represented by $C_p$ and 2) the cost of using samples, i.e. the sample size represented by $C_s$. 

\subsubsection{Solving Q1} 

Note that AQP++ and VAST can solve Q1 perfectly without sampling, i.e. $C_s$(AQP++) = $C_s$(VAST) = 0. Because of the tree-structure used by VAST, there's a $\rho_{h-1}$ chance that Q1 also aligns perfectly at layer $h-1$, and if that's the case, we have $C_p$(VAST) = $\frac{1}{\zeta} * C_p(AQP++)$. We can have the expected cost of solving Q1 using PA-tree.

\begin{figure}[h]
  \includegraphics[width=0.7\linewidth]{exp-figures/q1.png}
  \caption{Solving Q1}
  \label{fig:q1}
\end{figure}

% \[
% \mathop{\mathbb{E}}[C_p(VAST)] = \sum_{i=1}^{h-1}\rho_{i}\frac{1}{\zeta_{i}^{h-i}} C_p(AQP++)
% \]

% \xl{TODO: derive $\rho_i$}

\subsubsection{Solving Q2} 

To solve Q2 we have to utilize sampling to handle the $\Delta$, because of the PA-tree, to achieve the same $\Delta$, we have $C_p$(VAST) < $C_p$(AQP++). Take the advantage of stratified sampling, we have $C_s$(VAST) < $C_s$(AQP++) because AQP++ use uniform sampling.

\begin{figure}[h]
  \includegraphics[width=0.7\linewidth]{exp-figures/q2.png}
  \caption{Solving Q2}
  \label{fig:q2}
\end{figure}

\subsubsection{Solving Q3} 

For Q3, due to the PA-tree, the VAST baseline that traverse from the root only needs to expand the `edge' nodes that introduce $\Delta$, nodes in the center can remain un-expanded while still provide a perfect summary on the covered area. Therefore, we have $C_p$(VAST) $\le$ $C_p$(AQP++).

To use sampling to estimate $\Delta$, to achieve the best result, we assign all the samples to the leaf layer because the most fine-grain strata provides the best estimator. We have $C_s$(VAST) < $C_s$(AQP++) due to the advantage of stratified sampling.

Our best approach is called \textbf{VAST*}, i.e. a hybrid of PA Tree and an optimized stratified sampling approach. Our optimization includes: optimal sample assignment using variance; delta-encoding and what else??.

\begin{figure}[h]
  \includegraphics[width=0.7\linewidth]{exp-figures/q3.png}
  \caption{Solving Q3}
  \label{fig:q3}
\end{figure}

\subsection{US vs. ST vs. AQP++ vs. VAST}


\begin{figure}[h]
  \includegraphics[width=0.7\linewidth]{exp-figures/cnt.png}
  \caption{Median relative error of 100 COUNT queries given different sample rate}
  \label{fig:q3}
\end{figure}

\begin{figure}[h]
  \includegraphics[width=0.7\linewidth]{exp-figures/sum.png}
  \caption{Median relative error of 100 SUM queries given different sample rate}
  \label{fig:q3}
\end{figure}

% \begin{figure}[h]
%   \includegraphics[width=0.7\linewidth]{exp-figures/avg.png}
%   \caption{Median relative error of 100 AVG queries given different sample rate}
%   \label{fig:q3}
% \end{figure}

Our quantitative analysis utilize a PA-tree of 4 layers, we measure $C_p$(VAST) and $C_p$(AQP++) that can provide the best accuracy $\alpha_p$ and $\alpha_p < \alpha_t$. Then we gradually increase the sample rate and measure the overall accuracy of VAST and AQP++ (PA-Leaf + US in the figure).

\begin{figure*}
  \includegraphics[width=0.7\linewidth]{exp-figures/sel_vs_sr_LOSM.png}
  \caption{Median relative error of 2000 SUM queries break down by selectivity given different sample rate}
  \label{fig:sel}
\end{figure*}

% \begin{figure*}
%   \includegraphics[width=\textwidth]{figures/uml.png}
%   \caption{The UML diagram of the prototype.}
%   \label{fig:uml}
% \end{figure*}
\clearpage


\subsection{A Optimized Hybrid of Pre-aggregation and Stratified Sampling}
AQP++ combines PA and sampling by:
\[
Sol(Q) = PA(Q') + Sampling(Q) - Sampling(Q')
\]
Where $Q$ is the query we want to solve, and $Q'$ is the same query but with a predicate that is completely covered by Q and can be accurately solved by PA.

In our design, we can further optimize the query processing by utilizing the PA-guided strata in three ways:
1) we can safely avoid sampling from the irrelevant strata given the query predicates and 2) we can safely avoid sampling from  the strata that is completely covered by the query
3) we can safely avoid sampling from  the stratum with a variance of 0 because we can derive its result.

To do that, we need to find out the $\Delta Q$, which is the difference between Q and Q', then we solve the query by:
\[
Sol(Q) = PA(Q') + \sum_{q_i \in \Delta Q, \cup q_i = \Delta Q, \cap q_i = \emptyset }{Sampling(q_i)}
\]

Comparing with AQP++, this approach largely reduce the search space with the guidance of PA, which means a improved accuracy given the same sample size as shown in the \textbf{OptVAST} baseline in Figure \ref{fig:opt}. However, we need to find a explicit representation of $\Delta Q$, calculate up to $2N_d$ sub-queries where $N_d$ is the number of dimensions then combine the results, which introduces additional overhead.

\begin{figure*}
  \includegraphics[width=0.7\linewidth]{exp-figures/sr_vs_sel_Opt.png}
  \caption{Median relative error of 3000 SUM queries break down by selectivity given different sample rate. OptVAST is the optimized VAST that skips sampling from irrelevant and covered stratum.}
  \label{fig:opt}
\end{figure*}

\begin{figure*}
  \includegraphics[width=\textwidth]{figures/arch.png}
  \caption{The architecture of the system.}
  \label{fig:sampletree}
\end{figure*}



==> newApproxPart.tex <==
We propose a practical index such that given a bucket $\rho$ it returns a constant approximation to the query with the maximum variance in $\rho$ for $n_\rho\geq 2\delta n$.
For a query $q$ in bucket $\rho$, let $V_q=n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2$. Notice that the real variance of a SUM/COUNT query $q$ is $\sqrt{\frac{N_\rho^2}{n_\rho^3}V_q}$, while the real variance of an AVG query $q$ is $\sqrt{\frac{1}{n_\rho\cdot |q|^2}V_q}$.


We fist prove some useful properties we are going to use later.
\begin{lemma}
\label{lem1}
Let $q$ be a query in bucket $\rho$, where $|q|\leq \alpha n_\rho$, for a parameter $\alpha\leq 1$. Then it holds that $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2 \geq (1-\alpha)n_\rho \sum_{h\in q}t_h^2$.
\end{lemma}
\begin{proof}
We have $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2 = (n_\rho-1)\sum_{h\in q}t_h^2 - 2\sum_{i<j\in q}t_it_j = (n_\rho-|q|)\sum_{h\in q}t_h^2 + (|q|-1)\sum_{h\in q}t_h^2- 2\sum_{i<j\in q}t_it_j = (n_\rho-|q|)\sum_{h\in q}t_h^2 + \sum_{i<j\in q} (t_i-t_j)^2\geq (n_\rho-|q|)\sum_{h\in q}t_h^2 \geq (1-\alpha)n_\rho\sum_{h\in q}t_h^2$.
\end{proof}


\begin{lemma}
\label{lem2}
The AVG query with the largest variance $q$ contains less than $2\delta n$ sampled items, i.e., $|q|< 2\delta n$.
\end{lemma}
\begin{proof}
we show it by contradiction. Assume that this is not the case so $|q|\geq 2\delta n$. Let $q_L, q_R$ be queries with $|q_L|=|q_R|=|q|/2\leq n_\rho/2$, where the left boundary of $q_L$ is the same with the left boundary of $q$ and the right boundary of $q$ is the right boundary of $q$. Notice that $q=q_L\cup q_R$ and $q_L\cap q_R=\emptyset$. Without loss of generality $\sum_{h\in q_L}t_h^2\geq \sum_{h\in q_R}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$.

Since $q$ is the query with the largest variance we have $\frac{1}{|q|^2}[n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2]> \frac{1}{|q_L|^2}[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]\Leftrightarrow n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2> 4[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]$. Since $|q_L|\leq n_\rho/2$, from Lemma~\ref{lem1} we have that $4[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]\geq 2n_\rho\sum_{h\in q_L}t_h^2$. Recall that $\sum_{h\in q_L}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$ so we conclude that $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2>\sum_{h\in q}t_h^2$, which is a contradiction.
\end{proof}

\begin{lemma}
\label{lem3}
Let $q$ be the query with the largest variance in $\rho$ with $n_\rho\geq 2\delta n$.

For SUM and COUNT queries, if $|q|\leq n_\rho/2$ then for any parameter $1/2\leq \alpha\leq 1$ we have that $V_q\geq V_{q'}\geq \frac{1}{4}V_q$, where $q'$ is the query with the largest $\sum_{h\in q'}t_h^2$ among queries with length $\max\{\alpha\cdot |q|,\delta n\}$.

For SUM and COUNT queries, if $|q|> n_\rho/2$ then for any parameter $1/4\leq \alpha\leq 1/2$ we have that $V_q\geq V_{q'}\geq \frac{1}{8}V_q$, where $q'$ is the query with the largest $\sum_{h\in q'}t_h^2$ among queries with length $\max\{\alpha\cdot |q|,\delta n\}$.

For AVG queries, we have that $\frac{1}{|q|^2}V_q\geq \frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_q$, where $q'$ is the query with the largest $\sum_{h\in q'}t_h^2$ among queries with length $\delta n$.
\end{lemma}
\begin{proof}
We start by proving the first part of the lemma.
Let $q_L, q_R$ be queries with $|q_L|=|q_R|=\max\{\alpha\cdot |q|,\delta n\}\leq n_\rho/2$, where the left boundary of $q_L$ is the same with the left boundary of $q$ and the right boundary of $q$ is the right boundary of $q$. Notice that $q=q_L\cup q_R$. Without loss of generality let $\sum_{h\in q_L}t_h^2\geq \sum_{h\in q_R}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$, so we also have $\sum_{h\in q'}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$.
We have $n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2\geq n_\rho\sum_{h\in q'}t_h^2-(\sum_{h\in q'}t_h)^2$. Notice that $|q'|\leq n_\rho/2$ so from Lemma~\ref{lem1} $n_\rho\sum_{h\in q'}t_h^2-(\sum_{h\in q'}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in q'}t_h^2$. Recall that $\sum_{h\in q'}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$ so $\frac{n_\rho}{2}\sum_{h\in q'}t_h^2\geq \frac{n_\rho}{4}\sum_{h\in q}t_h^2\geq \frac{1}{4}[n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2]$, so we conclude that $V_q\geq V_{q'}\geq \frac{1}{4}V_q$.

Similarly, we can show the second part of the lemma. The only difference is that since $1/4\leq \alpha\leq 1/2$ we can get a query $\hat{q}$ with $\sum_{h\in \hat{q}}t_h^2\geq \frac{1}{4}\sum_{h\in q}t_h^2$ and the result follows.

The third part of the lemma also follows easily from the above cases and Lemma~\ref{lem2} but we show it for completeness. We know that the maximum variance query has length at most $2\delta n$. Hence, we can find at least one query $q_L\subseteq q$ with length $\delta n$ such that $\sum_{h\in q_L}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$, so $\sum_{h\in q'}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$. We have,
$\frac{1}{|q|^2}[n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2]\geq \frac{1}{|q'|^2}[n_\rho\sum_{h\in q'}t_h^2-(\sum_{h\in q'}t_h)^2]\geq \frac{1}{2|q'|^2}(n_\rho\sum_{h\in q'}t_h^2)\geq \frac{1}{4|q'|^2}(n_\rho\sum_{h\in q}t_h^2)=\frac{|q|^2}{4|q'|^2}\frac{1}{|q|^2}(n_\rho\sum_{h\in q}t_h^2)\geq \frac{|q|^2}{4|q'|^2}\frac{1}{|q|^2}[n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2]\geq \frac{1}{4}\frac{1}{|q|^2}V_q$. So $\frac{1}{|q|^2}V_q\geq \frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_q$.
\end{proof}

\mparagraph{Practical index}
%We start with some preprocessing. We first sort the sampled items in ascending order with respect to the constraint attribute $C$. We compute the prefix sums $Y[i]=\sum_{h\leq i}t_h$, $Z[i]=\sum_{h\leq i}t_h^2$.
We start with the preprocessing.
Let $\mathcal{I}=\{\delta n \cdot 2^j\mid j=0,\ldots, \log \frac{1}{\delta}\}$. Notice that $|\mathcal{I}|=O(\log n)$. For AVG queries we only use $\mathcal{I}=\{\delta n\}$. For each $i\in \mathcal{I}$ we do the following:
%For each sampled item $t_j$ we compute the value $p_j=\sum_{j-i+1\leq h\leq j}t_h^2$. Let $P^i$ be the set of these values. Notice that $P^i$ can be constructed in $O(n)$ time passing once over all the sampled items in ascending order and using the table $Z$.
We construct a binary search tree $T^i$ over the sampled items with respect to their constraint attribute. Given an interval $[l,r]$ we can use the tree $T^i$ to find a partition of the sampled items in $[l,r]$ with $O(\log n)$ subsets, in $O(\log n)$ time. Let $u$ be a node of $T^i$ and $T_u^i$ be the set of sampled items in the area (interval) of $u$ and let $n_u=|T_u^i|$. For a node $u$ we store the sample $t_g\in T_u^i$ with the largest value $\sum_{g-i+1\leq h\leq g}t_h^2$.

All samples with the largest values in a a tree $T^i$ can be computed in $O(n)$ time in a bottom-up way.
Overall, the index we construct has $O(n\log n)$ space and can be constructed in $O(n\log n)$ time for SUM/COUNT queries. For AVG queries the index has $O(n)$ space and can be constructed in $O(n)$ time.

Assume that we are given a bucket $\rho=[a,b]$ and we want to find the query with the maximum variance in it. For any $i\in \mathcal{I}$ with $i\leq n_\rho/2$ we do the following (for AVG queries we only consider $i=\delta n$). We run a search on $T^i$ using the interval $[a+i-1,b]$. Let $\mathcal{L}$ be the set of $O(\log n)$ canonical nodes of $T^i$ that cover all sampled items in $[a+i-1,b]$.
We store the sample $t_g$ with the largest value $\sum_{g-i+1\leq h\leq g}t_h^2$.
Finally, we return the sample $t_{g^*}$ with the largest value $\sum_{g^*-i+1\leq h\leq g^*}t_h^2$ among all $i\in \mathcal{I}$ with $\delta n\cdot 2^i\leq n_\rho/2$. Let $T^i$ be the tree that we found $t_{g^*}$. We report the query:  $q'=[t_{g^*-i+1}, t_{g^*}]$.

\begin{lemma}
The query time of the index for SUM and COUNT queries is $O(\log^2 n)$, while the query time for AVG queries is $O(\log n)$.
\end{lemma}
\begin{proof}
There are $O(\log n)$ possible trees $T^i$ for SUM and COUNT queries. For each tree we find $O(\log n)$ canonical nodes and we return the sample with the largest sum of squares value. The total query time is $O(\log^2 n)$ for SUM and COUNT queries and $O(\log n)$ for AVG queries.
\end{proof}

\begin{lemma}
\label{lem4}
Let $q$ be the query with the largest variance in $\rho$ and let $q'$ be the query returned by our algorithm. For SUM and COUNT queries, if $|q|\leq n_\rho/2$ then $V_{q'}\geq \frac{1}{4}V_{q}$, otherwise $V_{q'}\geq \frac{1}{8}V_{q}$. For AVG queries $\frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_{q}$.
\end{lemma}
\begin{proof}
For any $j$, our index finds the query $q^j$ with the largest value $\sum_{h\in q^j}t_h^2$. So our index considers all possible queries of length $\delta n 2^j$ and returns the one with the largest sum of squares value.

We start proving our lemma for SUM and COUNT queries. Assume that $|q|\leq n_\rho/2$. Let $j$ be the largest exponent such that $\delta n 2^j\leq |q|$. Notice that $\delta n 2^j=\alpha |q|\leq n_\rho/2$, for a parameter $\alpha$ such that $1/2\leq\alpha\leq 1$. Hence from the first part of Lemma~\ref{lem3} we have that $V_{q'}\geq \frac{1}{4}V_{q}$. Next, assume that $|q|> n_\rho/2$. Let $j$ be the largest exponent such that $\delta n 2^j\leq |q|$. If $j=0$ then this is similar to the previous case so we have the same result. If $j\geq 1$ we are not sure if $\delta n 2^j\leq n_\rho/2$. However, it holds that $\delta n 2^{j-1}\leq n_\rho/2$. In that case $\delta n 2^{j-1} = \alpha|q|$ for a parameter $\alpha$ such that $1/4\leq \alpha\leq 1/2$. Hence from the second part of Lemma~\ref{lem3} we have that $V_{q'}\geq \frac{1}{4}V_{q}$.

Last, we consider the AVG queries. It follows directly from Lemma~\ref{lem3} that $\frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_{q}$.
\end{proof}

Our practical index can be used with the DP algorithm to get a $4$-approximation partition for SUM and COUNT queries in $O(kn\log^2 n)$ time and a $2$-approximation partition for AVG queries in $O(kn\log n)$ time, in $1$d.


By extending the ideas above to higher dimensions we can get an index of $\Tilde{O}(n)$ space in $\Tilde{O}(n)$ such that given a rectangle $\rho$ it returns the a query $q'$ such that $V_{q'}\geq O(\frac{1}{n^{1-1/d}})V_q$, in $\Tilde{O}(\frac{1}{n^{1-1/d}})$ time. That leads 
to a DP algorithm to get a $O(n^{1-1/d})$-approximation partition for all SUM, COUNT and AVG queries in $\Tilde{O}(kn^{2-1/d})$ time, in $d$-dimensions. The $\Tilde{O}(\cdot)$ notation hides $\log n$ factors.







\stavros{Below is a proof that I mentioned in the previous version that if the intuition is not clear I will add it. It is about how an approximation $\AMAXV$ leads to an approximation for the DP problem. So I decided to write the proof here just for completeness.}
\begin{lemma}
Let $q'$ be the query returned by $\AMAXV$ such that $V_q'\geq \alpha V_{q^*}$, where $q^*$ is the query with the largest variance in a bucket $\rho$, and $\alpha<1$ be a parameter. Then the DP algorithm will return a partition $R$ such as $\max{q\in Q_R^1}error(q,R)\leq \frac{1}{\sqrt{\alpha}} \min_{R\in\mathcal{R}}\max_{q\in Q_R^1}error(q,R)$. The same holds using the ternary search.  
\end{lemma}
\begin{proof}
Let $A^*[i,j]$ be the optimum partition among the first $i$ items with $j$ buckets. Our DP finds $A[i,j]$ as an approximation of $A^*[i,j]$ for each $i, j$. We show by induction on $j$ that the partition found in $A[i,j]$ has variance at most $\frac{1}{\alpha}$ times the optimum variance $A^*[i,j]$.

We start the induction with the base case $j=2$.
Let the optimum partition with two buckets be $[1,h], [h+1, i]$ with maximum variance $V^*$. From the definition of $\AMAXV$ we have a value $V_1$ such that $V_1^*\geq V_1\geq \alpha V_1^*$, and a value $V_2$ such that $V_2^*\geq V_2\geq \alpha V_2^*$, where $V_1^*$ is the largest variance query in $[1,h]$ and $V_2^*$ is the largest variance query in $[h+1,i]$.
Assume that our approximation algorithm chooses to partition $[1,h'], [h'+1,i]$ with largest variance $V^{*'}$. Again, from the definition of $\AMAXV$ we have values $V_1', V_2'$ such that $V_1^{*'}\geq V_1'\geq \alpha V_1^{*'}$, $V_2^{*'}\geq V_2'\geq \alpha V_2^{*'}$, where $V_1^{*'}$ is the largest variance query in $[1,h']$ and $V_2^{*'}$ is the largest variance query in $[h'+1,i]$.
Since our algorithm chooses the second partition, it holds that $\max\{V_1',V_2'\}\leq \max\{V_1,V_2\}$. Without loss of generality assume that $V_1'\geq V_2'$. We have that $V_1'\leq \max\{V_1,V_2\}\leq \max\{V_1^*, V_2^*\}= V^*$. Furthermore, $V_1'\geq \alpha V_1^{*'}$ and $V_1'\geq V_2'\geq \alpha V_2^{*'}$. Hence, $V_1'\geq \alpha\max\{V_1^{*'}, V_2^{*'}\}=\alpha V^{*'}$. Overall, $\alpha V^{*'}\leq V_1'\leq V^*$. Similarly we can show that $\alpha V^{*'}\leq V_2'\leq V^*$ if $V_2'\geq V_1'$. Hence, in $A[i,2]$ we store a value $V'$ such that $\alpha V^{*'}\leq V'\leq V^*$. Hence, it also holds that $V^{*'}\leq\frac{1}{\alpha}V^*$.

Assume that for all $g<j$ it holds that $A[i,g]$ (for all $i$) has a value $V_{i,g}$ such as $\alpha V_{i,g}^{*'}\leq V_{i,g}\leq V_{i,g}^*$, where $V_{i,g}^*$ is the optimum partition among the first $i$ element with $g$ buckets and $V_{i,g}^{*'}$ is the maximum variance of a query in the computed partition for $A[i,g]$. We show that we can also argue the same for a partition $A[i,j]$ (for any $i$). Similarly to the previous case assume that the optimum partition with $j$ buckets among the first $i$ elements has the last bucket $[h+1,i]$. From the induction hypothesis we have that $\alpha V_{h,j-1}^{*'}\leq V_{h,j-1}\leq V_{h,j-1}^*$. Furthermore, from the definition of $\AMAXV$ we have $\alpha V_2^*\leq V_2\leq V_2^*$ for the bucket $[h+1,i]$, where $V^*2$ is the largest variance in $[h+1,i]$. If our algorithm chooses this partition the result follows. Assume that our algorithm chooses a different partition where the last bucket is $[h'+1, i]$. From the induction hypothesis we have $\alpha V_{h',j-1}^{*'}\leq V_{h',j-1}'\leq V_{h',j-1}^*$. Furthermore, from the definition of $\AMAXV$ we have $\alpha V_2^{*'}\leq V_2'\leq V_2^{*'}$ for the bucket $[h'+1,i]$, where $V_2^{*'}$ is the largest variance in $[h'+1,i]$. Since our algorithm does not choose the optimum partition we have $\max\{V_{h',j-1}',V_2'\}\leq \max\{V_{h,j-1},V_2\}$.
Without loss of generality $V_{h',j-1}'\geq V_2'$. We have $V_{h',j-1}'\leq \max\{V_{h,j-1},V_2\}\leq \max\{V_{h,j-1}^*,V_2^*\}=V_{i,j}^*$.
Furthermore, $V_{h',j-1}'\geq \alpha V_{h',j-1}^{*'}$, and $V_{h',j-1}'\geq V_2'\geq \alpha V_2^{*'}$ so $V_{h',j-1}'\geq \alpha \max\{V_{h',j-1}^{*'}, V_2^{*'}\}=\alpha V_{i,j}^{*'}$. Similarly we can show that $V_2'\leq V_{i,j}^*$ and $V_2'\geq\alpha V_{i,j}^{*'}$, if $V_2'\geq V_{h',j-1}'$. Hence in $A[i,j]$ we store a value $V_{i,j}'$ such that $\alpha V_{i,j}^{*'}\leq V_{i,j}'\leq V_{i,j}^*$.
So, it also holds that $V_{i,j}^{*'}\leq\frac{1}{\alpha}V_{i,j}^*$.

The error is defined taking the square roots of the variances we compute so the approximation ratio is $\frac{1}{\sqrt{\alpha}}$.

Similarly, we can show that these variants hold if we run the ternary search in the DP algorithm.
\end{proof}



\remove{We propose indexes such that given a bucket $\rho$ they return a constant approximation to the query with the maximum variance in $\rho$ for $n_\rho\geq 2\delta n$. The first index is more theoretical than the second one, however it has a better constant approximation factor.
For a query $q$ in bucket $\rho$, let $V_q=n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2$. Notice that the real variance of a SUM/COUNT query $q$ is $\sqrt{\frac{N_\rho^2}{n_\rho^3}V_q}$, while the real variance of an AVG query $q$ is $\sqrt{\frac{1}{n_\rho\cdot |q|^2}V_q}$.


We fist prove some useful properties we are going to use later.
\begin{lemma}
\label{lem1}
Let $q$ be a query in bucket $\rho$, where $|q|\leq \alpha n_\rho$, for a parameter $\alpha\leq 1$. Then it holds that $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2 \geq (1-\alpha)n_\rho \sum_{h\in q}t_h^2$.
\end{lemma}
\begin{proof}
We have $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2 = (n_\rho-1)\sum_{h\in q}t_h^2 - 2\sum_{i<j\in q}t_it_j = (n_\rho-|q|)\sum_{h\in q}t_h^2 + (|q|-1)\sum_{h\in q}t_h^2- 2\sum_{i<j\in q}t_it_j = (n_\rho-|q|)\sum_{h\in q}t_h^2 + \sum_{i<j\in q} (t_i-t_j)^2\geq (n_\rho-|q|)\sum_{h\in q}t_h^2 \geq (1-\alpha)n_\rho\sum_{h\in q}t_h^2$.
\end{proof}


\begin{lemma}
\label{lem2}
The AVG query with the largest variance $q$ contains less than $2\delta n$ sampled items, i.e., $|q|< 2\delta n$.
\end{lemma}
\begin{proof}
we show it by contradiction. Assume that this is not the case so $|q|\geq 2\delta n$. Let $q_L, q_R$ be queries with $|q_L|=|q_R|=|q|/2\leq n_\rho/2$, where the left boundary of $q_L$ is the same with the left boundary of $q$ and the right boundary of $q$ is the right boundary of $q$. Notice that $q=q_L\cup q_R$ and $q_L\cap q_R=\emptyset$. Without loss of generality $\sum_{h\in q_L}t_h^2\geq \sum_{h\in q_R}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$.

Since $q$ is the query with the largest variance we have $\frac{1}{|q|^2}[n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2]> \frac{1}{|q_L|^2}[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]\Leftrightarrow n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2> 4[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]$. Since $|q_L|\leq n_\rho/2$, from Lemma~\ref{lem1} we have that $4[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]\geq 2n_\rho\sum_{h\in q_L}t_h^2$. Recall that $\sum_{h\in q_L}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$ so we conclude that $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2>n_\rho\sum_{h\in q}t_h^2$, which is a contradiction.
\end{proof}

\begin{lemma}
\label{lem3}
Let $q$ be the query with the largest variance in $\rho$ with $n_\rho\geq 2\delta n$.

For SUM and COUNT queries, if $|q|\leq n_\rho/2$ then for any parameter $1/2\leq \alpha\leq 1$ we have that $V_q\geq V_{q'}\geq \frac{1}{4}V_q$, where $q'$ is the query with the largest variance among queries with length $\max\{\alpha\cdot |q|,\delta n\}$.

For SUM and COUNT queries, if $|q|> n_\rho/2$ then for any parameter $1/4\leq \alpha\leq 1/2$ we have that $V_q\geq V_{q'}\geq \frac{1}{8}V_q$, where $q'$ is the query with the largest variance among queries with length $\max\{\alpha\cdot |q|,\delta n\}$.

For AVG queries, we have that $\frac{1}{|q|^2}V_q\geq \frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_q$, where $q'$ is the query with the largest variance among queries with length $\delta n$.
\end{lemma}
\begin{proof}
We start by proving the first part of the lemma.
Let $q_L, q_R$ be queries with $|q_L|=|q_R|=\max\{\alpha\cdot |q|,\delta n\}\leq n_\rho/2$, where the left boundary of $q_L$ is the same with the left boundary of $q$ and the right boundary of $q$ is the right boundary of $q$. Notice that $q=q_L\cup q_R$. Without loss of generality let $\sum_{h\in q_L}t_h^2\geq \sum_{h\in q_R}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$.
We have $n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2\geq n_\rho\sum_{h\in q_L}t_h^2-(\sum_{h\in q_L}t_h)^2$. Notice that $|q_L|\leq n_\rho/2$ so from Lemma~\ref{lem1} $n_\rho\sum_{h\in q_L}t_h^2-(\sum_{h\in q_L}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in q_L}t_h^2$. Recall that $\sum_{h\in q_L}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$ so $\frac{n_\rho}{2}\sum_{h\in q_L}t_h^2\geq \frac{n_\rho}{4}\sum_{h\in q}t_h^2\geq \frac{1}{4}[n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2]$, so we conclude that $V_q\geq V_{q_L}\geq \frac{1}{4}V_q$. Notice that $V_{q'}\geq V_{q_L}$ and $V_{q'}\leq V_q$ so we conclude that $V_q\geq V_{q'}\geq \frac{1}{4}V_q$.

Similarly, we can show the second part of the lemma. The only difference is that since $1/4\leq \alpha\leq 1/2$ we can get a query $\hat{q}$ with $\sum_{h\in \hat{q}}t_h^2\geq \frac{1}{4}\sum_{h\in q}t_h^2$ and the result follows.

The third part of the lemma also follows easily from the above cases and Lemma~\ref{lem2} but we show it for completeness. We know that the maximum variance query has length at most $2\delta n$. Hence, we can find at least one query $q_L\subseteq q$ with length $\delta n$ such that $\sum_{h\in q_L}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$. We have,
$\frac{1}{|q|^2}[n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2]\geq \frac{1}{|q_L|^2}[n_\rho\sum_{h\in q_L}t_h^2-(\sum_{h\in q_L}t_h)^2]\geq \frac{1}{2|q_L|^2}(n_\rho\sum_{h\in q_L}t_h^2)\geq \frac{1}{4|q_L|^2}(n_\rho\sum_{h\in q}t_h^2)=\frac{|q|^2}{4|q_L|^2}\frac{1}{|q|^2}(n_\rho\sum_{h\in q}t_h^2)\geq \frac{|q|^2}{4|q_L|^2}\frac{1}{|q|^2}(n_\rho\sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2)\geq \frac{1}{4}\frac{1}{|q|^2}V_q$. So $\frac{1}{|q|^2}V_q\geq \frac{1}{|q_L|^2}V_{q_L}\geq \frac{1}{4}\frac{1}{|q|^2}V_q$. Since $|q_L|=|q'|=\delta n$, it follows that $\frac{1}{|q|^2}V_q\geq \frac{1}{|q'|^2}V_{q'}\geq \frac{1}{|q_L|^2}V_{q_L}$, so $\frac{1}{|q|^2}V_q\geq \frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_q$.
\end{proof}

\mparagraph{Theoretical index}
We start with some preprocessing. We first sort the sampled items in ascending order with respect to the constraint attribute $C$. We compute the prefix sums $Y[i]=\sum_{h\leq i}t_h$, $Z[i]=\sum_{h\leq i}t_h^2$.

Let $\mathcal{I}=\{\delta n \cdot 2^j\mid j=0,\ldots, \log \frac{1}{\delta}\}$. Notice that $|\mathcal{I}|=O(\log n)$. For AVG queries we only use $\mathcal{I}=\{\delta n\}$. For each $i\in \mathcal{I}$ we do the following:
For each sampled item $t_j$ we construct the $2$-dimensional point $p_j=(\sum_{j-i+1\leq h\leq j}t_h^2, (\sum_{j-i+1\leq h\leq j}t_h)^2)$. Let $P^i$ be the set of two dimensional points. Notice that $P^i$ can be constructed in $O(n)$ time passing once over all the sampled items in ascending order and using the tables $X, Z$.
We construct a binary search tree $T^i$ over the sampled items with respect to their constraint attribute. Given an interval $[l,r]$ we can use the tree $T^i$ to find a partition of the sampled items in $[l,r]$ with $O(\log n)$ subsets, in $O(\log n)$ time. Let $u$ be a node of $T^i$ and $T_u^i$ be the set of sampled items in the area (interval) of $u$ and let $n_u=|T_u^i|$. Let $P_u^i$ be the corresponding set of $2$-dimensional points in $T_u^i$. For node $u$ we construct a top-$1$ index\cite{} $\mathcal{D}_u^i$ over the points $P_u^i$. The index $\mathcal{D}_u^i$ has $O(n_u)$ space and given a two dimensional vector $v$ it returns $\argmax_{p\in P_u^i}\langle v,p\rangle$, i.e., the point in $P_u^i$ with the largest inner product with vector $v$. The query time on $\mathcal{D}_u^i$ is $O(\log n_u)$ \cite{}.
Overall, the index we construct has $O(n\log^2 n)$ space and can be constructed in $O(n\log^3 n)$ time for SUM/COUNT queries. For AVG queries the index has $O(n\log n)$ space and can be constructed in $O(n\log^2 n)$.

Assume that we are given a bucket $\rho=[a,b]$ and we want to find the query with the maximum variance in it. For any $i\in \mathcal{I}$ with $i\leq n_\rho/2$ we do the following (for AVG queries we only consider $i=\delta n$). We run a search on $T^i$ using the interval $[a+i-1,b]$. Let $\mathcal{L}$ be the set of $O(\log n)$ canonical nodes of $T^i$ that cover all sampled items in $[a+i-1,b]$. Let $v=(n_\rho, -1)$ be a $2$ dimensional vector. For each node $u\in \mathcal{L}$ we use the the index $\mathcal{D}_u^i$ to search for the point in $P_u^i$ with the largest inner product with respect to vector $v$. In the end we store the point $p^i$ with the largest inner product among all the nodes in $\mathcal{L}$. Finally, we return the point with the largest inner product among all $i\in \mathcal{I}$ with $\delta n\cdot 2^i\leq n_\rho/2$. Let $p_j$ be the point we return from tree $i$. We report that the query with the largest variance is $q'=[t_{j-i+1}, t_j]$.

\begin{lemma}
The query time of the index for SUM and COUNT queries is $O(\log^3 n)$, while the query time for AVG queries is $O(\log^2 n)$.
\end{lemma}
\begin{proof}
There are $O(\log n)$ possible trees $T^i$ for SUM and COUNT queries. For each tree we find $O(\log n)$ canonical nodes and for each node we run a top-$1$ query that takes $O(\log n)$ time. The total query time is $O(\log^3 n)$ for SUM and COUNT queries and $O(\log^2 n)$ for AVG queries.
\end{proof}

\begin{lemma}
\label{lem4}
Let $q$ be the query with the largest variance in $\rho$ and let $q'$ be the query returned by our algorithm. For SUM and COUNT queries, if $|q|\leq n_\rho/2$ then $V_{q'}\geq \frac{1}{4}V_{q}$, otherwise $V_{q'}\geq \frac{1}{8}V_{q}$. For AVG queries $\frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_{q}$.
\end{lemma}
\begin{proof}
For any $j$, our index finds the query with the largest variance and length $\delta n 2^j$. This is true because the inner product of a point $p_h$ with the vector $v=(n_\rho,-1)$ for $i=\delta n 2^j$ is equal to $V_{\bar{q}}$, where $\bar{q}=[t_{h-i+1}, t_h]$. So our index considers all possible queries of length $\delta n 2^j$ and returns the one with the largest variance.

We start proving our lemma for SUM and COUNT queries. Assume that $|q|\leq n_\rho/2$. Let $j$ be the largest exponent such that $\delta n 2^j\leq |q|$. Notice that $\delta n 2^j=\alpha |q|\leq n_\rho/2$, for $1/2\leq\alpha\leq 1$. Hence from the first part of Lemma~\ref{lem3} we have that $V_{q'}\geq \frac{1}{4}V_{q}$. Next, assume that $|q|> n_\rho/2$. Let $j$ be the largest exponent such that $\delta n 2^j\leq |q|$. If $j=0$ then this is similar to the previous case so we have the same result. If $j\geq 1$ we are not sure if $\delta n 2^j\leq n_\rho/2$. However, it holds that $\delta n 2^{j-1}\leq n_\rho/2$. In that case $\delta n 2^{j-1} = \alpha|q|$ for $1/4\leq \alpha\leq 1/2$. Hence from the second part of Lemma~\ref{lem3} we have that $V_{q'}\geq \frac{1}{8}V_{q}$.

Last, we consider the AVG queries. It follows directly from Lemma~\ref{lem3} that $\frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q|^2}V_{q}$.
\end{proof}

Our theoretical index can be used with the DP algorithm to get a $4$-approximation partition for SUM and COUNT queries in $O(kn\log^4 n)$ time and a $2$-approximation partition for AVG queries in $O(kn\log^3 n)$ time, in $1$d.

\mparagraph{Practical index}
The index we proposed in the previous section is not very practical due to the top-$1$ index we need to construct. The main reason that we need such an index is that the variance of a query $q$ depends on the number of elements of the bucket that it belongs to. For example, if $\rho_1, \rho_2$ are two buckets that both contain a query $q$ the variance of $q$ with respect to $\rho_1$ will be different than the variance with respect to bucket $\rho_2$. In particular, the issue is the term $n_\rho \sum_{h\in q}t_h^2$, since different $n_\rho$ should be multiplied with $\sum_{h\in q}t_h^2$. Notice that the rest normalizing factors $N_\rho$, or $n_\rho$ in front of $V_q$ do not play any important role because all queries in a bucket $\rho$ are multiplied with these factors.

In order to solve this issue without performing a top-$1$ query we consider a few different values of $n_\rho$. In particular we construct the following simpler to implement index.
As we had before, let $\mathcal{I}=\{\delta n \cdot 2^j\mid j=0,\ldots, \log \frac{1}{\delta}\}$. For AVG queries we only use $\mathcal{I}=\{\delta n\}$.
Let $\mathcal{W}=\{2\delta n 2^j\mid j=0,\ldots, \log\frac{1}{2\delta}\}$. As we did before, for any $i\in \mathcal{I}$ we construct the set of $2$ dimensional points $P^i$. For any pair $i\in \mathcal{I}, w\in \mathcal{W}$, we construct the search binary tree $T^{i,w}$ over the constraint attributes of the sampled items. Let $u$ be a node in $T^{i,w}$ and let $T^{i,w}_u$ be the sampled items in the range (interval) of node $u$. Let $v=(w,-1)$ be a vector. In node $u$ we store the sample $t_u=\argmax_{t_h\in T^{i,w}_u} \langle v, p_h\rangle$. In other words, in the node $u$ of the tree $T^{i,w}$ we store a query $q$ that has the following properties: i) it has length $i$, ii) it has its right boundary in the interval that corresponds to the node $u$, and iii) it has the largest value $w\cdot \sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2$.
In total we construct $O(\log^2 n)$ trees and each tree has size $O(n)$. Hence, our index for SUM and COUNT queries has $O(n\log^2 n)$ space and it can be constructed in $O(n\log^2 n)$ time. The index for AVG queries has $O(n\log n)$ space and can be constructed in $O(n\log n)$ time.

Assume that we are given a bucket $\rho=[a,b]$ and our goal is to find a query that approximates the query with the largest variance in $\rho$. Let $j$ be the value such that $2\delta n 2^j< n_\rho\leq 2\delta n 2^{j+1}$, and let $w=2\delta n 2^{j+1}$. For any $i\in \mathcal{I}$ with $i\leq n_\rho/2$ (for AVG we only consider $i=\delta n$) we run a search in $T^{i,w}$ on the interval $[a+i-1, b]$. In that way we return the query $q_{i,w}$ whose right endpoint belongs in $[a+i-1,b]$, with length $i$, that maximizes $w\sum_{h\in q_{i,w}}t_h^2 - (\sum_{h\in q_{i,w}}t_h)^2$. We repeat the same for all $i\in \mathcal{I}$ with $i\leq n_\rho/2$ and in the end we choose the query with the largest value $w\sum_{h\in q_{i,w}}t_h^2 - (\sum_{h\in q_{i,w}}t_h)^2$, among all $i$ we consider.

\begin{lemma}
The query time of our index is $O(\log^2 n)$ for SUM and COUNT queries and $O(\log n)$ for AVG queries.
\end{lemma}
\begin{proof}
For SUM and COUNT queries we search over $O(\log n)$ trees ($O(\log n)$ different values of $i$) and each search takes $O(\log n)$ time. For AVG we only search over one tree. The query times follow.
\end{proof}

\begin{lemma}
Let $q$ be the query with the largest variance in bucket $\rho$ and let $q'$
be the query returned by our practical index.
It holds that $V_q'\geq \frac{1}{24}V_q$ for SUM and COUNT queries and $V_q'\geq \frac{1}{12}V_q$ for AVG queries.
\end{lemma}
\begin{proof}
Let $1\leq \beta\leq 2$ be a parameter. For any query $\bar{q}$ with $|\bar{q}|\leq n_\rho/2$ it holds that $n_\rho \sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2 \leq \beta n_\rho \sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2\leq 3[n_\rho \sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2]$. The first inequality is obvious. We prove the second inequality. We have
$\beta n_\rho \sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2\leq n_\rho \sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2 + n_\rho \sum_{h\in \bar{q}}t_h^2$. From Lemma~\ref{lem1} we know that $n_\rho\sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in \bar{h}} t_h^2$ so we conclude that $\beta n_\rho \sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2\leq 3[n_\rho \sum_{h\in \bar{q}}t_h^2 - (\sum_{h\in \bar{q}}t_h)^2]$.

Let $q_1$ be the query returned by our practical index and let $q_2$ be the query that would return if we could search for the maximum variance for the real $n_\rho$ value, i.e., $q_2$ is the query returned by the theoretical index. Recall that $w/2< n_\rho\leq w$. Hence, $w=\beta n_\rho$ for a parameter $1<\beta\leq 2$.
From our observation above we have $\beta n_\rho\sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1})^2\leq 3[n_\rho\sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1})^2]$. We also know that $\beta n_\rho\sum_{h\in q_2}t_h^2 - (\sum_{h\in q_2})^2\geq n_\rho\sum_{h\in q_2}t_h^2 - (\sum_{h\in q_2})^2$. Notice that our practical index considers the query $q_2$ since the values $\mathcal{I}$ that the practical and theoretical index try are the same.
Since our practical index returns $q_1$ and not $q_2$ we have $\beta n_\rho\sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1})^2\geq \beta n_\rho\sum_{h\in q_2}t_h^2 - (\sum_{h\in q_2})^2$.
Overall, $n_\rho\sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1})^2\geq \frac{1}{3}[\beta n_\rho\sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1})^2]\geq \frac{1}{3}[\beta n_\rho\sum_{h\in q_2}t_h^2 - (\sum_{h\in q_2})^2]\geq \frac{1}{3}[n_\rho\sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1})^2]$. From Lemma~\ref{lem4} recall that in the worst case $V_{q_2}\geq \frac{1}{8}V_q$ for SUM and COUNT queries and $\frac{1}{|q_2|^2}V_{q_2}\geq \frac{1}{4}\frac{1}{|q|^2}V_q$ for AVG queries. We conclude that $V_{q_1}\geq \frac{1}{24}V_q$ for SUM and COUNT queries and $\frac{1}{|q_1|^2}V_{q_1}\geq \frac{1}{12}\frac{1}{|q|^2}V_{q}$ for AVG queries.
\end{proof}


Our practical index can be used with our DP algorithm to get a $4\sqrt{3}$-approximation partition for SUM and COUNT queries in $O(kn\log^3 n)$ time and a $2\sqrt{3}$-approximation partition in $O(kn\log^2 n)$ time, in $1$d.

Unfortunately, these indexes cannot be extended in higher dimensions easily.







\stavros{Below is a proof that I mentioned in the previous version that if the intuition is not clear I will add it. It is about how an approximation $\AMAXV$ leads to an approximation for the DP problem. So I decided to write the proof here just for completeness.}
\begin{lemma}
Let $q'$ be the query returned by $\AMAXV$ such that $V_q'\geq \alpha V_{q^*}$, where $q^*$ is the query with the largest variance in a bucket $\rho$, and $\alpha<1$ be a parameter. Then the DP algorithm will return a partition $R$ such as $\max{q\in Q_R^1}error(q,R)\leq \frac{1}{\sqrt{\alpha}} \min_{R\in\mathcal{R}}\max_{q\in Q_R^1}error(q,R)$. The same holds using the ternary search.  
\end{lemma}
\begin{proof}
Let $A^*[i,j]$ be the optimum partition among the first $i$ items with $j$ buckets. Our DP finds $A[i,j]$ as an approximation of $A^*[i,j]$ for each $i, j$. We show by induction on $j$ that the partition found in $A[i,j]$ has variance at most $\frac{1}{\alpha}$ times the optimum variance $A^*[i,j]$.

We start the induction with the base case $j=2$.
Let the optimum partition with two buckets be $[1,h], [h+1, i]$ with maximum variance $V^*$. From the definition of $\AMAXV$ we have a value $V_1$ such that $V_1^*\geq V_1\geq \alpha V_1^*$, and a value $V_2$ such that $V_2^*\geq V_2\geq \alpha V_2^*$, where $V_1^*$ is the largest variance query in $[1,h]$ and $V_2^*$ is the largest variance query in $[h+1,i]$.
Assume that our approximation algorithm chooses to partition $[1,h'], [h'+1,i]$ with largest variance $V^{*'}$. Again, from the definition of $\AMAXV$ we have values $V_1', V_2'$ such that $V_1^{*'}\geq V_1'\geq \alpha V_1^{*'}$, $V_2^{*'}\geq V_2'\geq \alpha V_2^{*'}$, where $V_1^{*'}$ is the largest variance query in $[1,h']$ and $V_2^{*'}$ is the largest variance query in $[h'+1,i]$.
Since our algorithm chooses the second partition, it holds that $\max\{V_1',V_2'\}\leq \max\{V_1,V_2\}$. Without loss of generality assume that $V_1'\geq V_2'$. We have that $V_1'\leq \max\{V_1,V_2\}\leq \max\{V_1^*, V_2^*\}= V^*$. Furthermore, $V_1'\geq \alpha V_1^{*'}$ and $V_1'\geq V_2'\geq \alpha V_2^{*'}$. Hence, $V_1'\geq \alpha\max\{V_1^{*'}, V_2^{*'}\}=\alpha V^{*'}$. Overall, $\alpha V^{*'}\leq V_1'\leq V^*$. Similarly we can show that $\alpha V^{*'}\leq V_2'\leq V^*$ if $V_2'\geq V_1'$. Hence, in $A[i,2]$ we store a value $V'$ such that $\alpha V^{*'}\leq V'\leq V^*$. Hence, it also holds that $V^{*'}\leq\frac{1}{\alpha}V^*$.

Assume that for all $g<j$ it holds that $A[i,g]$ (for all $i$) has a value $V_{i,g}$ such as $\alpha V_{i,g}^{*'}\leq V_{i,g}\leq V_{i,g}^*$, where $V_{i,g}^*$ is the optimum partition among the first $i$ element with $g$ buckets and $V_{i,g}^{*'}$ is the maximum variance of a query in the computed partition for $A[i,g]$. We show that we can also argue the same for a partition $A[i,j]$ (for any $i$). Similarly to the previous case assume that the optimum partition with $j$ buckets among the first $i$ elements has the last bucket $[h+1,i]$. From the induction hypothesis we have that $\alpha V_{h,j-1}^{*'}\leq V_{h,j-1}\leq V_{h,j-1}^*$. Furthermore, from the definition of $\AMAXV$ we have $\alpha V_2^*\leq V_2\leq V_2^*$ for the bucket $[h+1,i]$, where $V^*2$ is the largest variance in $[h+1,i]$. If our algorithm chooses this partition the result follows. Assume that our algorithm chooses a different partition where the last bucket is $[h'+1, i]$. From the induction hypothesis we have $\alpha V_{h',j-1}^{*'}\leq V_{h',j-1}'\leq V_{h',j-1}^*$. Furthermore, from the definition of $\AMAXV$ we have $\alpha V_2^{*'}\leq V_2'\leq V_2^{*'}$ for the bucket $[h'+1,i]$, where $V_2^{*'}$ is the largest variance in $[h'+1,i]$. Since our algorithm does not choose the optimum partition we have $\max\{V_{h',j-1}',V_2'\}\leq \max\{V_{h,j-1},V_2\}$.
Without loss of generality $V_{h',j-1}'\geq V_2'$. We have $V_{h',j-1}'\leq \max\{V_{h,j-1},V_2\}\leq \max\{V_{h,j-1}^*,V_2^*\}=V_{i,j}^*$.
Furthermore, $V_{h',j-1}'\geq \alpha V_{h',j-1}^{*'}$, and $V_{h',j-1}'\geq V_2'\geq \alpha V_2^{*'}$ so $V_{h',j-1}'\geq \alpha \max\{V_{h',j-1}^{*'}, V_2^{*'}\}=\alpha V_{i,j}^{*'}$. Similarly we can show that $V_2'\leq V_{i,j}^*$ and $V_2'\geq\alpha V_{i,j}^{*'}$, if $V_2'\geq V_{h',j-1}'$. Hence in $A[i,j]$ we store a value $V_{i,j}'$ such that $\alpha V_{i,j}^{*'}\leq V_{i,j}'\leq V_{i,j}^*$.
So, it also holds that $V_{i,j}^{*'}\leq\frac{1}{\alpha}V_{i,j}^*$.

The error is defined taking the square roots of the variances we compute so the approximation ratio is $\frac{1}{\sqrt{\alpha}}$.

Similarly, we can show that these variants hold if we run the ternary search in the DP algorithm.
\end{proof}
}

==> newApproxPart2.tex <==
\section{Practical algorithms with provable guarantees}
In this section we propose some very simple algorithms for computing an approximation of the maximum variance in a rectangular area for SUM, COUNT and AVG queries.
In particular, given a bucket $\rho$ in $\Re^d$ for constant $d$, we propose efficient approximations to the query with the maximum variance in $\rho$ for $n_\rho\geq 2\delta n$.
For a query $q$ in bucket $\rho$, let $V_q=n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2$. Notice that the length of the confidence interval of a SUM/COUNT query $q$ depends on $\sqrt{\frac{N_\rho^2}{n_\rho^3}V_q}$, while the length of the confidence interval of an AVG query $q$ depends on $\sqrt{\frac{1}{n_\rho\cdot |q|^2}V_q}$.
Finding an approximation to the maximum $V_q$ in $\rho$ leads to an efficient approximation algorithm for minimizing the length of the confidence interval.


We fist prove a useful lemma we are going to use later.
\begin{lemma}
\label{lem1}
Let $q$ be a query in bucket $\rho$, where $|q|\leq \alpha n_\rho$, for a parameter $\alpha\leq 1$. Then it holds that $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2 \geq (1-\alpha)n_\rho \sum_{h\in q}t_h^2$.
\end{lemma}
\begin{proof}
We have $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2 = (n_\rho-1)\sum_{h\in q}t_h^2 - 2\sum_{i<j\in q}t_it_j = (n_\rho-|q|)\sum_{h\in q}t_h^2 + (|q|-1)\sum_{h\in q}t_h^2- 2\sum_{i<j\in q}t_it_j = (n_\rho-|q|)\sum_{h\in q}t_h^2 + \sum_{i<j\in q} (t_i-t_j)^2\geq (n_\rho-|q|)\sum_{h\in q}t_h^2 \geq (1-\alpha)n_\rho\sum_{h\in q}t_h^2$.
\end{proof}


First, we propose an algorithm for SUM and COUNT queries and then we solve the AVG query for any constant dimension $d$.
\renewcommand{\O}{\widetilde{O}}
\subsection{SUM and COUNT queries}
Before we describe our algorithm we execute some preprocessing so we can compute efficiently $\sum_{h\in q}t_h^2$ or $\sum_{h\in q}t_h$ for a rectangular query $q$. In $1$-dimension we just compute the prefix sums $X[i]=\sum_{h\leq i}t_h^2$ and $Y[i]=\sum_{h\leq i}t_h$. In higher dimensions we construct a range tree in $\O(n)$ time that has space $\O(n)$. Given a a query rectangle $q$ the range tree can return $\sum_{h\in q}t_h^2$ and $\sum_{h\in q}t_h$ in $\O(1)$ time. The notation $\O(\cdot)$ hides $\log n$ factors.

\mparagraph{Algorithm}
Let $\rho$ be a rectangle in $\Re^d$. By finding the median item (in any dimension), we split $\rho$ into two queries $q_1, q_2$ such that $q_1\cup q_2=\rho$, $q_1\cap q_2=\emptyset$ and $|q_1|=|q_2|=n_\rho/2$. If $\sum_{h\in q_1}t_h^2\geq \sum_{h\in q_2}t_h^2$ then we return the variance $V_{q_1}$, otherwise we return $V_{q_2}$.

\mparagraph{Running time}
After the preprocessing our algorithm runs in $O(1)$ time for $1$-dimension and $\O(1)$ in any constant dimension $d$.


\mparagraph{Correctness}
We show the following lemma.
\begin{lemma}
\label{proof1}
Let $V_{q_1}$ be the variance that our algorithm returns and let $V_{q^*}$ be the maximum variance. Then $V_{q_1}\geq \frac{1}{4}V_{q^*}$.
\end{lemma}
\begin{proof}
First, notice that $|q_1|=n_\rho/2$ so from Lemma~\ref{lem1} we have $V_{q_1}=n_\rho \sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in q_1}t_h^2$.
Second, notice that $\sum_{h\in q_1}t_h^2\geq \frac{1}{2}\sum_{h\in q^*}t_h^2$. This holds because: If $q^*\subseteq q_1$ or $q^*\subseteq q_2$ then $\sum_{h\in q_1}t_h^2\geq \sum_{h\in q_2}t_h^2\geq \sum_{h\in q^*}t_h^2$. If $q^*$ intersects both of $q_1$ and $q_2$ then $\max\{\sum_{h\in q_1}t_h^2, \sum_{h\in q_2}t_h^2\}\geq \frac{1}{2}\sum_{h\in q^*}t_h^2$.

Hence we conclude that $V_{q_1}=n_\rho\sum_{h\in q_1}t_h^2 - (\sum_{h\in q_1}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in q_1}t_h^2\geq \frac{1}{4}n_\rho\sum_{h\in q^*}t_h^2\geq \frac{1}{4}[n_\rho\sum_{h\in q^*}t_h^2 - (\sum_{h\in q^*}t_h)^2]=\frac{1}{4}V_{q^*}$.
\end{proof}

If our algorithm is used with the DP algorithm in $1$-dimension it gives a $2\sqrt{2}$-approximation of the total error in $O(kn\log n)$ time.
If our algorithm is used with the k-d tree for any constant dimension $d$ it gives a $2\sqrt{k}$-approximation with respect to the class of k-d trees in $\O(n+k)$ time.



\subsection{AVG queries}

We first show an important property for AVG queries.
\begin{lemma}
\label{lemAVG}
The AVG query with the largest variance $q$ contains less than $2\delta n$ sampled items, i.e., $|q|< 2\delta n$.
\end{lemma}
\begin{proof}
we show it by contradiction. Assume that this is not the case so $|q|\geq 2\delta n$. Let $q_L, q_R$ be queries with $|q_L|=|q_R|=|q|/2\leq n_\rho/2$, where the left boundary of $q_L$ is the same with the left boundary of $q$ and the right boundary of $q$ is the right boundary of $q$. Notice that $q=q_L\cup q_R$ and $q_L\cap q_R=\emptyset$. Without loss of generality $\sum_{h\in q_L}t_h^2\geq \sum_{h\in q_R}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$.

Since $q$ is the query with the largest variance we have $\frac{1}{|q|^2}[n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2]> \frac{1}{|q_L|^2}[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]\Leftrightarrow n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2> 4[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]$. Since $|q_L|\leq n_\rho/2$, from Lemma~\ref{lem1} we have that $4[n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2]\geq 2n_\rho\sum_{h\in q_L}t_h^2$. Recall that $\sum_{h\in q_L}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$ so we conclude that $n_\rho\sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2>\sum_{h\in q}t_h^2$, which is a contradiction.
\end{proof}

Using the fact that we can focus only on queries that contain at most $2\delta n$ items we design two algorithms. The first one works in $1$-dimension and the second one works in any constant dimension $d$.

First, we have the same preprocessing as in the SUM and COUNT queries.

\mparagraph{Algorithm for $1$-dimension}
We construct a binary search tree $T$ over the sampled items with respect to their constraint attribute. Given an interval $[l,r]$ we can use the tree $T$ to find a partition of the sampled items in $[l,r]$ with $O(\log n)$ subsets, in $O(\log n)$ time. Let $u$ be a node of $T$ and $T_u$ be the set of sampled items in the area (interval) of $u$ and let $n_u=|T_u|$. For a node $u$ we store the sample $t_g\in T_u$ with the largest value $\sum_{g-\delta n+1\leq h\leq g}t_h^2$.

All samples with the largest values in each node of $T$ can be computed in $O(n)$ time in a bottom-up way.
Overall, the index we construct has $O(n)$ space and can be constructed in $O(n)$ time.

Assume that we are given a bucket $\rho=[a,b]$ and we want to find the query with the maximum variance in it. We run a search on $T$ using the interval $[a+\delta n-1,b]$. Let $\mathcal{L}$ be the set of $O(\log n)$ canonical nodes of $T$ that cover all sampled items in $[a+\delta n-1,b]$.
We get the sample $t_g$ with the largest value $\sum_{g-\delta n+1\leq h\leq g}t_h^2$ among all nodes in $\mathcal{L}$.
We return query $q'=[t_{g-\delta n+1}, t_{g}]$ with variance $V_{q'}$.

\paragraph{Running time}
After the preprocessing we can construct the tree in $O(n)$ time. Given bucket $\rho$ we return $q'$in $O(\log n)$ time.


\paragraph{Correctness}
We show the next lemma.
\begin{lemma}
\label{lem:AVG}
Let $q^*$ be the query with the largest variance in $\rho$ and let $q'$ be the query returned by our algorithm. It holds that $\frac{1}{|q'|^2}V_{q'}\geq \frac{1}{4}\frac{1}{|q^*|^2}V_{q^*}$.
\end{lemma}
\begin{proof}
Our index finds the query $q'$ with the largest value $\sum_{h\in q'}t_h^2$ among all queries in $\rho$ with length $\delta n$.
Since $n_\rho\geq 2\delta n$ we have that $|q'|\leq n_\rho/2$ so from Lemma~\ref{lem1} $n_\rho\sum_{h\in q'}t_h^2 - (\sum_{h\in q'}t_h)^2\geq  \frac{n_\rho}{2}\sum_{h\in q'}t_h^2$. In addition, notice that $\sum_{h\in q'}t_h^2\geq \frac{1}{2}\sum_{h\in q^*}t_h^2$, since $|q^*|<2\delta n$ and we can always get two queries (intervals) with length $\delta n$ completely inside $\rho$ that cover $q^*$. Hence, similarly to Lemma~\ref{proof1} we get:
$\frac{1}{|q'|^2}{V_{q'}}=\frac{1}{|q'|^2}[n_\rho\sum_{h\in q'}t_h^2 - (\sum_{h\in q'}t_h)^2]\geq \frac{1}{|q'|^2}\frac{n_\rho}{2}\sum_{h\in q'}t_h^2\geq \frac{1}{|q'|^2}\frac{1}{4}n_\rho\sum_{h\in q^*}t_h^2\geq \frac{|q^*|^2}{4|q'|^2}\frac{1}{|q^*|^2}[n_\rho\sum_{h\in q^*}t_h^2 - (\sum_{h\in q^*}t_h)^2]\geq \frac{1}{4}\frac{1}{|q^*|^2}V_{q^*}$.
\end{proof}

If our algorithm is used with the DP algorithm it gives a $2$-approximation of the total error in $1$-dimension in $O(kn\log^2 n)$ time.


\mparagraph{Algorithm in $d$-dimensions}
For simplicity we describe the algorithm in $2$-dimensions, however it can be generalized to any dimension. Let $\rho$ be a rectangle in $2$-d.
We project all sampled points $t$ on the $y$ axis and we sort them with respect to $y$.
We also sort the points with respect to the $x$ coordinate.
For each item $t$ in $\rho$ we do the following: Let $w=2^i$ for integer $i=0,\ldots, \log n$. Let $t'$ be the $w$-th point below $t$ with respect to the $y$ coordinate. We run a binary search (using the range trees for counting queries) with respect to the $x$ axis to the right side of $t.x$ to find the item $\hat{t}$ such that the rectangle defined by the opposite corners $(t.x, t.y)\times (\hat{t}.x, t'.y)$ contains exactly $\delta n$ points. Similarly, we find the point $\bar{t}$ at the left side of $t.x$ such that the rectangle defined by the opposite corners $(\bar{t}.x, t.y)\times (t.x, t'.y)$ contains exactly $\delta n$ points. If there is not such a rectangle that contain $\delta n$ points (this can happen if there are not enough items in $\rho$ to get such a rectangle) then we proceed as follows: Without loss of generality assume that there is not such rectangle at the right side of $t.x$. Then let $\tilde{t}$ be the item with the largest $x$ coordinate. By running binary search we find the item $\hat{t}$ at the left side of $t.x$ such that the rectangle defined by the opposite corners $(\hat{t}.x, t.y)\times(\tilde{t}.x,t'.y)$ contains $\delta n$ items. If such rectangle does not exist then let $\hat{t}$ be the item with the smallest $x$ coordinate. By running binary search over the $y$ coordinates we find the item $p$ such that the rectangle defined by the opposite corners $(\hat{t}.x,t.y)\times(\tilde{t}.x, p.y)$ has $\delta n$ items. If such rectangle does not exist we skip $t$ and we continue with the next item.
For each item $t$ we also repeat the symmetric process above $t.y$, .i.e, considering the $w=2^i$-th item above $t.y$ for integer $i=0,\ldots, \log n$.
Among all rectangles we process, we store and update the rectangle $q$ with the largest value $\sum_{h\in q}t_h^2$ (given a rectangle $q$ this value can be found in $\O(1)$ time running a query in the range tree).
In the end, among all the $\O(n)$ rectangles we processed, we return the rectangle (query) $q'$ with the largest value $\sum_{h\in q'}t_h^2$.


\mparagraph{Running time}
For each point in $\rho$ we spend $\O(1)$ time so in total our algorithm runs in $\O(n)$ time.

\mparagraph{Correctness}
The next lemma is a direct geometric property of the rectangles we process during the algorithm.
\begin{lemma}
\label{lem:part}
Let $R$ be the set of all valid rectangles we consider as we run our algorithm. For any rectangle $H\subseteq \rho$ (including the rectangle corresponding to the query with the largest variance) there is a set of rectangles $A_1,\ldots, A_s$, where $s=O(1)$, such that $A_i\in R$ for each $i\leq s$ and $\bigcup_{i\leq s}A_i\supseteq H$.
\end{lemma}

We conclude with the next lemma.
\begin{lemma}
Let $q^*$ be the query with the largest variance in $\rho$ and $q'$ the query returned by our algorithm. It holds that $\frac{1}{|q'|^2}V_{q'}\geq \frac{1}{O(1)}\frac{1}{|q^*|^2}V_{q^*}$.
\end{lemma}
\begin{proof}
Notice that all rectangles considered by our algorithm contain $\delta n$ items. From Lemma~\ref{lem:part} we know that there exists a set of $s=O(1)$ rectangles $A_1,\ldots, A_s$ such that $\bigcup_{i\leq s}A_i\supseteq q^*$. Let $A_{i^*}$ be the rectangle with the largest value $\sum_{h\in A_{i^*}} t_h^2$. We have that $\sum_{h\in q'}t_h^2\geq \sum_{h\in A_{i^*}} t_h^2 \geq \frac{1}{O(1)}\sum_{h\in q^*}t_h^2$. Using our new observations and the steps of the proof of Lemma~\ref{lem:AVG} it follows that $\frac{1}{|q'|^2}V_{q'}\geq \frac{1}{O(1)}\frac{1}{|q^*|^2}V_{q^*}$.
\end{proof}


If our algorithm is used with the k-d tree it gives a $O(1)$-approximation of the total error in any constant dimension $d$ with respect to the class of k-d trees in $\O(kn)$ time.

==> oldproof.tex <==
All the algorithms we proposed so far compute the query with the maximum variance in a range $[i, j]$ by considering all possible queries in $[i,j]$. In the worst case the function $\MAXV([i,j])$ can be computed in $O(|Q|)$ time, where $|Q|=O(m^2)$. Hence, the algorithm might not be practical in large datasets. Here, we propose a way to compute an approximation of $\MAXV[i,j]$ more efficiently. We call this function $\AMAXV$.

The high level idea is the following: We divide the $j-i+1$ samples into smaller groups. In order to find the query with the largest variance we consider all possible queries with  respect to the boundaries of the smaller groups. In the end we show that if groups are small enough we can get an approximation of the query with largest variance.

We first start by introducing some useful notation.
Let $\Gamma=\frac{\max_{j}t_j}{\min_{j: t_j>0}t_j}$ be the spread of the values of the non-zero sampled items.
Without changing the result of our algorithm we scale all aggregate values of the sampled items such that $\min_{j: t_j>0}t_j=1$ and $\max_{j}t_j=\Gamma$.
Notice that for binary values of the tuples $t$ (for example in COUNT queries), $\Gamma=1$.
%Notice that these are reasonable assumptions since each bucket and query should contain sufficient number of sampled points in order to be able to have a reasonable estimation of the variance.

We are ready to describe our new procedure for computing $\AMAXV(\rho)$, for an interval $\rho$.
Let $\eps$ be a parameter such that $\delta\leq \eps\leq \frac{1}{2\Gamma}$.
We divide the samples in $\rho$ to $L=\frac{1}{\eps}$ groups such that each group contains $\eps n_\rho$ items. Let $G_\rho=g_1,\ldots, g_{L+1}$ be the $L+1$ boundaries of the sampled points. For each pair $g_u, g_v\in G$ we compute the variance of the query $[g_u, g_v]$. In the end we return the maximum variance over all possible queries defined by $G$.


Using the pre-computed values of $X, Y, Z$ we described above, $\AMAXV$ runs in $O(\frac{1}{\eps^2})$ time.

Next we show that the result returned by our new procedure is close to the variance of the query with the maximum  variance in $\rho$.
For simplicity, we assume that $\delta\ll \frac{1}{2\Gamma}$.
We focus on the case where $n_\rho\geq 2\Gamma\delta n$, i.e., the bucket does not have very small size.
Hence, each group we construct has at least $\delta n$ sampled items.
We can get almost similar results for the case $n_\rho<2\Gamma\delta n$.
\stavros{This case is a harder corner case and I'm still working to see what is the best we can have for this one. But I don't think this special case ($n_\rho<2\Gamma\delta n$) is so important to mention it here. UPDATE: I found a way to handle this case as well. The proof holds for any $n_\rho\geq 2\delta n$ so I might update the current proof we have to a new maybe more elegant proof.}

We show the approximation factor for the AVG query, which is the most complicated one, and in the end we show how to extend to SUM and COUNT queries.
Let $q$ be the query (interval) with the largest variance in $\rho$. If the boundaries of $q$ lie on $G$ then our method returns the query with the largest variance.



Next, assume that $q$ fully contains at least one group and partially intersects two (or one) groups. In particular let $q=q_L\cup q_C \cup q_R$, where $q_L$ is the left part of the query that partially intersects a group, $q_C$ is the part of the query that fully contains a few (at least one) groups, and $Q_R$ is the right part of the query that partially intersects a group. Then we have $V_{q}=\frac{1}{n_{\rho,q}^2}[n_\rho\sum_{h\in q} t_h^2 - (\sum_{h\in q} t_h)^2]$ (we skip the factors $\frac{1}{n_\rho})$ \zs{thinking about giving it a name so  we could reuse it. also easier for the readers to understand what's going on}that is the same for any possible query in the bucket $\rho$. We have
$\frac{1}{n_{\rho,q}^2}[n_\rho \sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2] \leq \frac{1}{n_{\rho,q}^2}[n_\rho \sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2 +n_\rho \sum_{h\in q_C}t_h^2 - (\sum_{h\in q_C}t_h)^2+n_\rho \sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R}t_h)^2]$.
We consider two cases. If $n_\rho \sum_{h\in q_C}t_h^2 - (\sum_{h\in q_C}t_h)^2 \geq \max\{n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2, n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R}t_h)^2\}$ then $V_{q}\leq \frac{3}{n_{\rho,q_C}^2}[n_\rho\sum_{h\in q_C}t_h^2 - (\sum_{h\in q_C}t_h)^2]$ so $\frac{1}{n_{\rho,q_C}^2}[n_\rho\sum_{h\in q_C}t_h^2 - (\sum_{h\in q_C}t_h)^2]\geq \frac{1}{3}V_{q}$. Notice that $q_C$ is a query that we always consider in  our algorithm since its endpoints lie in $G$. Hence in this case we will return a $1/3$ approximation of the maximum variance.

The second case we consider is when 
$n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R}t_h)^2 \geq \max\{n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2, n_\rho\sum_{h\in q_C}t_h^2 - (\sum_{h\in q_C}t_h)^2\}$ (equivalently we can consider that $q_L$ has the largest value, but the idea is the same).
Let $I_R$ be the group of sampled items that contains $q_R$. We show that the variance of $I_R$ is close to the variance of $V_q$.
Recall that $n_{\rho,I_R}\geq \delta n$, so it is a valid query.
The variance of $I_R$ is defined as (skipping the normalizing factors)  $\frac{1}{n_{\rho, I_R}^2}[n_\rho\sum_{h\in I_R}t_h^2 - (\sum_{h\in I_R} t_h)^2]$.
Before we continue we need to show the following technical lemma.

\begin{lemma}
\label{lem:techn}
Let $q', \hat{q}$ be two queries in bucket $\rho$ such that $q'$ is contained in $\hat{q}$ with $n_{\rho,q'}<n_{\rho,\hat{q}}\leq \eps n_\rho\leq \frac{1}{2\Gamma}n_\rho$. It holds that $n_\rho\sum_{h\in q'}t_h^2- (\sum_{h\in q'}t_h)^2\leq n_\rho\sum_{h\in \hat{q}}t_h^2- (\sum_{h\in \hat{q}}t_h)^2$.
\end{lemma}
\begin{proof}
Let $\bar{q}=q'\cup\{x\}$ be a query in $\rho$ that contains query $q'$ along with one more sampled item $x$.
If $x=0$ then it follows that $n_\rho\sum_{h\in \bar{q}} t_h^2 -(\sum_{h\in \bar{q}})^2= n_\rho\sum_{h\in q'} t_h^2 -(\sum_{h\in q'})^2$. Next, we assume that $x>0$.
We have $n_\rho\sum_{h\in \bar{q}} t_h^2 -(\sum_{h\in \bar{q}})^2=n_\rho\sum_{h\in q'}t_h^2-(\sum_{h\in q'}t_h)^2 +x[(n_\rho-1)x-2\sum_{h\in q'}t_h]$.
Notice that $\frac{2\sum_{h\in q'}t_h}{x}\leq 2(\eps n_\rho-1)\Gamma\leq  2\Gamma(\frac{n_\rho}{2\Gamma}-1)\leq n_\rho-1$.
% \zs{where does this -1 from the first inequality come from?}
% \stavros{When we state the lemma, we say that the size of query $q'$ is $<\eps n_\rho$ so I wrote it as $\leq \eps n_\rho-1$ since the size of $q'$ is integer and assuming that $\eps n_r\rho$ is an integer (we can take slightly larger $\eps$ to make it integer if $\eps n_\rho$ is not integer). However, I slightly changed it to make more clear.}
From the last inequality we have $n_\rho\geq \frac{2\sum_{h\in q'}t_h}{x}+1\Leftrightarrow (n_\rho-1)x-2\sum_{h\in p'} t_h\geq 0$. 
% \zs{is LHS an assumption?} \stavros{No, the LHS is exactly what we have in the previous inequality. I can write everything in one sentence to make it clear} 
It follows that $n_\rho\sum_{h\in \bar{q}} t_h^2 -(\sum_{h\in \bar{q}})^2\geq n_\rho\sum_{h\in q'} t_h^2 -(\sum_{h\in q'})^2$. By repeating the same argument for each new sampled item recursively we conclude that $n_\rho\sum_{h\in q'}t_h^2- (\sum_{h\in q'}t_h)^2\leq n_\rho\sum_{h\in \hat{q}}t_h^2- (\sum_{h\in \hat{q}}t_h)^2$.
\end{proof}
Notice that $n_{\rho, I_R}\leq \frac{n_\rho}{2\Gamma}$ and $q_R$ is contained in $I_R$, so
from Lemma~\ref{lem:techn} we showed that $\frac{1}{n_{\rho, I_R}^2}[n_\rho\sum_{h\in I_R}t_h^2 - (\sum_{h\in I_R} t_h)^2]\geq \frac{1}{n_{\rho, I_R}^2}[n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R} t_h)^2]$. Recall that $n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R}t_h)^2$ is at least $\max\{n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2, n_\rho\sum_{h\in q_C}t_h^2 - (\sum_{h\in q_C}t_h)^2\}$ so we have
$\frac{1}{n_{\rho, I_R}^2}[n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R} t_h)^2]\geq \frac{1}{3}\frac{1}{n_{\rho, I_R}^2}[n_\rho \sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L}t_h)^2 +n_\rho \sum_{h\in q_C}t_h^2 - (\sum_{h\in q_C}t_h)^2+n_\rho \sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R}t_h)^2]\geq \frac{1}{3}\frac{1}{n_{\rho, I_R}^2}[n_\rho \sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2]$. Since $n_{\rho, I_R}\leq n_{\rho, q}$ we have that $\frac{1}{n_{\rho, I_R}^2}[n_\rho\sum_{h\in I_R}t_h^2 - (\sum_{h\in I_R} t_h)^2]\geq \frac{1}{3}V_q$.

Finally, there is one more case to consider. Assume that the query with the maximum variance in $\rho$ does not completely contain any group. Let $q$ be the query with the maximum variance that partially intersects two consecutive groups (the case where the query lies completely inside a group is similar so we skip it). Let $q=q_L\cup q_R$, where $q_L$, $q_R$ is the part of the query in the left and right group, respectively. Without loss of generality we assume that $n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R} t_h)^2\geq n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L} t_h)^2$. We have $V_q=\frac{1}{n_{\rho, q}^2}[n_\rho \sum_{h\in q}t_h^2 - (\sum_{h\in q}t_h)^2]\leq \frac{1}{n_{\rho,q}^2}[n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R} t_h)^2 + n_\rho\sum_{h\in q_L}t_h^2 - (\sum_{h\in q_L} t_h)^2]\leq \frac{2}{n_{\rho,q}^2}[n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R} t_h)^2]$. Let $I_R$ be the interval (query) that defines the group of part $q_R$, so $q_R\subset I_R$. From Lemma~\ref{lem:techn} we have that $\frac{2}{n_{\rho,q}^2}[n_\rho\sum_{h\in q_R}t_h^2 - (\sum_{h\in q_R} t_h)^2] \leq \frac{2}{n_{\rho,q}^2}[n_\rho\sum_{h\in I_R}t_h^2 - (\sum_{h\in I_R} t_h)^2]$. Notice that $n_{\rho,q}\geq \delta m$, so $V_q\leq \frac{2}{\delta^2 m^2}[n_\rho\sum_{h\in I_R}t_h^2 - (\sum_{h\in I_R} t_h)^2]\leq\\ \frac{2\eps^2n_\rho^2}{\delta^2 m^2}\frac{1}{n_{\rho,I_R}^2}[n_\rho\sum_{h\in I_R}t_h^2 - (\sum_{h\in I_R} t_h)^2]\leq \frac{2\eps^2n_\rho^2}{\delta^2 m^2} V_{I_R} \Leftrightarrow V_{I_R}\geq \frac{\delta^2 m^2}{2\eps^2n_\rho^2}V_q$.
In the worse case $n_\rho\leq m$ so $V_{I_R}\geq \frac{\delta^2}{2\eps^2}V_q$.
%Notice that $I_R$ is one of the queries that our method considers we have that in this case we would get a $2(\Gamma\delta)^2$ approximation of the query with the maximum variance.

Overall, we conclude that $\AMAXV$ runs in $O(\frac{1}{\eps^2})$ time, and finds a query in a range $\rho$ with variance at least $1/3$ of the maximum variance, if the query with the largest variance is long enough, or (in the worst case) at least $\frac{\delta^2 m^2}{2\eps^2n_\rho^2}\geq \frac{\delta^2}{2\eps^2}$ if the query with the largest variance is short enough.
We note that if we set $\eps=\frac{\delta m}{n_\rho}$ we can get $\frac{1}{3}$-approximation in $O(\frac{1}{\delta^2})$ time.

So far we considered the AVG query. The results are better for SUM and COUNT queries since we do not have the factor $\frac{1}{n_{\rho,q}}$ that we need to approximate. Hence, for SUM and COUNT queries we can get $\frac{1}{3}$-approximation of the maximum variance in $O(\Gamma^2)$ time (notice that there is no reason to choose $\eps<\frac{1}{2\Gamma}$).


By replacing $\MAXV$ with $\AMAXV$ in the DP algorithm we get the recursion
$A[i,j]=\min_{h<i}\max\{A[h,j-1], \AMAXV([h+1,i])\}$. The new DP algorithm runs in $O(km\log(m)\frac{1}{\eps^2})$ time.
By skipping some low level details we can show that \stavros{If the intuition is not very clear , if needed and we have space, I can add the full proof (how an $\frac{1}{\alpha}$-approx for $\MAXV$ gives an $\alpha$-approx for the our problem using the DP)}
%for a cell $A[i,j]$, the approximated value $V$ found by the DP algorithm, using $\AMAXV$, satisfies $\frac{1}{\alpha}V'\leq V\leq V^*$, where $V^*$ is the variance of the optimum partition in $A[i,j]$, $V'$ is the real variance of the partition found by the DP algorithm, and $\alpha$ is the approximation ratio of finding the query with the maximum variance in an interval $[h,i]$. \stavros{I can add the full proof if is needed and we have space.} Hence, we can show that
our new algorithm finds a partition where the maximum variance query is at most $3$ times or $2(\frac{\eps}{\delta})^2$ times the maximum variance query of the optimum partition for AVG queries.
Alternatively, we can run the DP algorithm in $O(km\log(m)\frac{1}{\delta^2})$ time and find a partition where the maximum variance query is at most $3$ times the maximum variance query of the optimum partition for AVG queries.
For SUM or COUNT queries the DP runs in  $O(km\log(m)\Gamma^2)$ time and returns a partition where the maximum variance query is at most $3$ times the maximum variance query of the optimum partition.

==> optimization.backup.0929.tex <==
\section{Optimizing the Partitioning}
This section describes how we optimize PASS to meet a desired error rate.

\subsection{Objective and Search Space}
The first step is to process the user specified time constraints $\tau_c$ and $\tau_q$ into internal parameters.
As before, we consider a dataset $P$, where there is an aggregation column $A$, and a collection of predicate columns ($C_1,..,C_d$).
We calculate the maximum number of leaf nodes $k$ (which governs construction time) allowable in the time limit $\tau_c$.
Each leaf will define a rectangular partitioning conditions $x_i\leq C_i\leq y_i$ for $1\leq i\leq d$.
Then, we calculate the maximum number of samples per partition $n$ allowable in the time limit $\tau_q$.
The search space $\mathcal{T}$ is all PASS data structures with $k$ leaves and $n$ samples per leaf with a fixed fanout of $2^d$.

Next, we have to define a class of queries $Q$ that we care about.
While in general SQL predicates can be arbitrary, we restrict our self to a large class of ``sensible'' predicates.
Over this schema, we define Q to be AVG/SUM/COUNT queries in a ``rectangular regions'', which return the average value with respect to the attribute $A$ among all tuples with $x_i\leq C_i\leq y_i$ for $1\leq i\leq d$.
Our optimization framework can also support other definitions for $Q$ (hereafter called templates), but for brevity we will focus on rectangular averages.

Given this definition of $Q$ and $\mathcal{T}$, now we describe the optimization objective.
For a query $q\in Q$ let $T$ be the set of leaf nodes, and $T_q$ be the set of leaf nodes that partially intersect with the query predicate, we get an error formula as follows:
\[error(q,T)=\lambda\sqrt{\sum_{R \in T_q} w_R^2 \cdot V_{R}(q) }.\]
Note from the previous section, the structure of the leaf nodes governs the estimation error of the data structure. The shape of the tree (height and fanout) only affects construction time and query latency. 
Thus, it is sufficient to optimize PASS in two steps to control for worst-case query error: first choose an optimal partitioning of the leaf nodes, and then construct the full tree with a bottom up aggregation.
The core is algorithm is then to optimize the following ``flat'' partitioning:
\[R^*= \argmin_{ T \in \mathcal{T}_{leaves} } \max_{q\in Q} error(q,T).\]

\subsection{Non-Trivial Overlap Assumption}
Under mild assumptions, we can greatly simplify the optimization problem by considering only the queries that partially overlap with a single partition. This, however, requires an assumption that the partial overlaps are non-trivial (there actually exist tuples in the intersection of the query predicate and the partition). 

\vspace{0.5em}
\noindent \textbf{Non-Trivial Overlap Assumption. } Let $b\in R$ be a partition. Let $n_b$ be the number of sampled items in bucket $b$.
We assume that the valid queries of $Q$ with respect to a partitioning $R$, are the queries that intersect sufficiently many sampled points in each bucket that they partially intersect. Precisely, for a bucket $b\in R_q$, if $n_{q,b}$ is the number of sampled items in bucket $b$ that are contained in $q$, then we assume that $n_{q,b}\geq \delta n$.
\vspace{0.5em}

Basically, the assumption states that we only care about queries that meaningfully overlap when they do partially overlap.
Accordingly, we can define the set of ``meaningful'' queries with respect to a partitioning $R$ as $Q'=\{q\in Q\mid n_{q,b}\geq \delta n, \forall b\in R_q\}$~\footnote{We shorthand this as just $Q$ for the rest of the paper.}.
One can think of this set as rectangles whose boundaries are grounded with actual tuples in the dataset.
With this assumption there are not infinite queries to consider and we can define $|Q|$ as the number of different meaningful queries with respect to a sample of data. For example if two queries $q_1,q_2\in Q$ contain the same set of sampled points we count them as one query. If $Q$ is the set of all possible queries in $R^1$ then $|Q|=O(n^2)$. Generally, if $Q$ is the set of all possible queries in $R^d$ then $|Q|=O(n^{2d})$. 


With this assumption, we map Equation \ref{eq:main} to a simpler problem:

\begin{lemma}
\label{lem:Obs}
Let $Q_R^1\subseteq Q$ be the set of meaningful queries in $Q$ that intersect only one partition in partitioning $R$, and let $i_q$ be that partition.
We define a new problem, as:
\[R'=\argmin_{R\in \mathcal{R}} \max_{q\in Q_R^1}V_{i_q}(q).\]
It holds that%$R'$ is an optimal solution for the original problem:
\[\max_{q\in Q}error(q,R')\leq \sqrt{k}\min_{R\in \mathcal{R}}\max_{q\in Q} error(q,R),\]
for SUM and COUNT queries and 
\[\max_{q\in Q}error(q,R')=\min_{R\in \mathcal{R}}\max_{q\in Q} error(q,R),\]
for AVG queries.
\end{lemma}
\begin{proof}
Let $q'$ be the query with $error(q',R')=\max_{q\in Q}error(q,R')$ and let $N_{q'}$ be the total size of buckets in $R'$ that intersect with $q'$. Furthermore, let $V'=\max_{q\in Q_{R'}^1}V_{i_q}(q)$.
Since $q'$ is a valid query in $R'$, we have
$$error(q',R')=\lambda\sqrt{\sum_{b\in R_{q'}'}w_b^2V_b(q')}\leq \left(\sqrt{\sum_{b\in R_{q'}'}w_b^2}\right) \left(\lambda \sqrt{V'}\right)$$

%\frac{1}{N_{q'}^2}\sum_{b\in R_{q'}'}N_b^2V_b(q')\leq \frac{\sum_{b\in R_{q'}'}N_b^2}{N_{q'}^2}V'\leq V'.$$

Let $R^*$ be the optimum partition for Problem 1 and let $V^*=\max_{q\in Q_{R^*}^1}V_{i_{q}}(q)$. We note that $V'\leq V^*$, otherwise $R'$ would not be the optimum partition for Problem 2.
Finally, we have $V^*\leq \max_{q\in Q}error(q,R^*)=\min_{R\in \mathcal{R}}\max_{q\in Q}error(q,R)$,
because $V^*$ corresponds to the variance of a valid query with respect to partition $R^*$, and $w_b=1$ for all type of queries if a query is fully contained in one bucket. Hence, the maximum error in partition $R^*$ will always be at least $\lambda\sqrt{V^*}$.

Overall,
$\max_{q\in Q}error(q,R')\leq \left(\sqrt{\sum_{b\in R_{q'}'}w_b^2}\right) \min_{R\in \mathcal{R}}\max_{q\in Q}error(q,R)$.
For SUM and COUNT queries all weights are equal to $1$. In the worst case $q'$ partially intersects $k$ buckets of partition $R'$ so $\max_{q\in Q}error(q,R')\leq \sqrt{k} \min_{R\in \mathcal{R}}\max_{q\in Q}error(q,R)$.
For AVG queries it holds that $\sum_{b\in R_{q'}'}w_b^2\leq 1$, so 
$\max_{q\in Q}error(q,R')\leq\min_{R\in \mathcal{R}}\max_{q\in Q}error(q,R)$, and hence it follows that $\max_{q\in Q}error(q,R')=\min_{R\in \mathcal{R}}\max_{q\in Q}error(q,R)$.
\end{proof}
% \zs{let's both check that this extends to high dimension.}
% \stavros{In this sub-section 4.1, I did not make any assumption on the dimension. Everything holds in any dimension. For example, the way the proof is written does not assume $d=1$. It holds for any dimension because it just talks about “partition” and “queries” where both notions are defined in any dimension.}
\zs{this proof needs some rewriting. I feel this is too dense. let's label the equations that will be referred later, and refer them when we do}

From Lemma~\ref{lem:Obs} we have that
any optimum solution for Problem 2 is also optimum for Problem 1 for AVG queries and it is a $\sqrt{k}$-approximation for SUM and COUNT queries.
In addition, any $\alpha$-approximation algorithm for Problem 2 is also a $\alpha$-approximation for Problem 1 for AVG queries and a $\sqrt{k}\cdot\alpha$-approximation for SUM and COUNT queries. Notice that it is much easier to handle Problem 2 since we can find the query with the maximum error with respect to a partition $R$ by looking only on queries that are fully contained in buckets $b\in R$.

Notice that for AVG queries $$V_b(q)=\frac{1}{n_b}\cdot\frac{1}{n_{b,q}^2}\left[n_b\sum_{h\in q}t_h^2 - \left(\sum_{h\in q} t_h\right)^2\right],$$
while for SUM queries
$$V_b(q)=\frac{1}{n_b}\cdot\frac{N_b^2}{n_{b}^2}\left[n_b\sum_{h\in q}t_h^2 - \left(\sum_{h\in q} t_h\right)^2\right].$$
For COUNT queries the formula for $V_b(q)$ is identical to the formula for SUM queries with $t_h=1$.
Since we focus on queries that lie completely inside a bucket, for simplicity, in the next subsections we assume that the error of a query $q$ in bucket $b$ is $V_b(q)$ and not $\lambda\sqrt{V_b(q)}$. This does not change the solution to the problem.

%We use the AVG query which is the most complicated one, however all our results extend to SUM or COUNT queries. We always mention when a result for SUM or COUNT is different (they can actually only be better).

%Next, we propose an optimum algorithm for Problem 2 (and hence optimum for Problem 1) in $1$ dimension and we show a number of improvements. Furthermore, we present a faster approximation algorithm.
%In the end, we give an algorithm for constructing a partition in any dimension $d$ which is optimum assuming that the partition has a specific geometric structure.

\subsection{$1$-d Optimal Partitioning Algorithm}
\label{sec:dp_algo}
The key subroutine in the optimization phase is to find a partitioning that minimizes the maximum query variance.
First, let's consider the $1$-d case, where we simply have a collection of tuples $P = \{(c_i, a_i)\}_{i=1}^N$.
All meaningful rectangular queries over this collection will have predicate intervals defined by the $c_i$---in fact, there are $\mathcal{O}(N^2)$ such intervals.



\zs{here we miss a lot of assumptions. we have discussed them over the phone but they need to appear on the paper somewhere. for example, we first generate a sample then we look for a partition on the sample (i.e., not an iterative process)}
\stavros{Yes, I agree we need some assumptions here. That's why we said maybe to have another section before this one explaining the high level ideas of our techniques. We can have that discussion about samples etc in such a section or here}
We describe a dynamic programming algorithm assuming that the boundaries of the buckets can only be placed on the sampled tuples.
In the end we give the high level idea on how to extend the algorithm to handle cases where the boundaries can be placed in any position. After finding an optimum partition with $k$ buckets we construct a binary balanced search tree over the $k$ buckets as leaf nodes.

Before we start describing the algorithm we note that Lemma~\ref{lem:Obs} gives a $\sqrt{2}$ approximation for SUM and COUNT queries in $1$-d because a query can partially intersect at most $2$ buckets.

\newcommand{\MAXV}{\mathcal{M}}
\newcommand{\AMAXV}{\overline{\mathcal{M}}}
We first sort the samples in ascending order with respect to the attribute $C$.
We define the DP table $A$ of $n$ rows and $k$ columns. Let $A[i,j]$ be the optimum solution of Problem 2 among the first $i$ samples with at most $j$ buckets. \zs{at most or exactly}\stavros{Well, first I wrote exactly but then I changed it to at most. It doesn’t matter too much but with “at most” we don’t have “null” values in the DP array. As, I said it doesn’t matter too much so we can decide.} The solution to Problem 2 is found by $A[n,k]$.
Let $\MAXV$ be function that takes as input an interval $[i_1,i_2]$ and returns the maximum variance of a query $q\in Q$ that lie completely inside $[i_1,i_2]$.
Using the function $\MAXV$ we can define the recursion
$$A[i,j]=\min_{h<i}\max\{A[h,j-1], \MAXV([h+1,i])\}.$$
Notice that we can easily solve the base cases $A[i,1]$, $A[1,j]$ using the $\MAXV$ function.
\stavros{Here I didn't use any constraint on the number of samples in a bucket. We can assume if we want that the number of samples in a bucket is at least $\beta n$ for a parameter $\beta<1$, however in that case I am not sure about the main argument in paragraph "Improving the running time"}

Before we describe the $\MAXV$ function we do some preprocessing. We visit each item $t$ in the database and by running a binary search over the sorted samples we can find 
the sampled points $t_i, t_{i+1}$ such that $t_i\leq t\leq t_{i+1}$ with respect to the attribute $C$. Let $X[i]$ be the number of database items with value at most $t_i$. Similarly we construct prefix sums storing the sum of the values of the sampled points along with their sum of squares. Let $Y[i]=\sum_{g=1}^i t_g$ and $Z[i]=\sum_{g=1}^i t_g^2$.
After precomputed these values we are ready to describe the $\MAXV$ function.

Assume that we want to compute $\MAXV(h+1,i)$. If $i-h<\delta n$ we return $0$.
Otherwise, for any pair $g,w$ such that $h+1\leq g< w \leq i$ and $w-g+1\geq \delta n$
we compute the variance of the interval query $[g,w]$ in the bucket $[h+1, i]$. The exact calculation of the variance depends on the type of the query (AVG, SUM, COUNT) but it can always be computed in  $O(1)$ time assuming that we have the arrays $X, Y, Z$.
For example, the variance for AVG queries is computed as
$\frac{1}{i-h}\frac{1}{(w-g+1)^2}[(i-h)(Z[w]-Z[g-1])-(Y[w]-Y[g-1])^2]$.
%$\frac{1}{i-h}(1-\frac{i-h}{X[i]-X[h]})(\frac{i-h}{(w-g+1)^2}(Z[w]-Z[g-1])-\frac{1}{(w-g+1)^2}(Y[w]-Y[g-1])^2)$
We repeat the same for all pairs in $g<w\in [h+1, i]$ and we find the query with the maximum  variance.


From the definition of the DP recursion  algorithm returns $\min_{R\in\mathcal{R}}\max_{q\in Q}error(q,P)$, assuming that boundaries of the buckets are always on the sampled points. By storing the boundaries of the partition, the dynamic algorithm can also return the partition $R$ with the minimum error.


Notice that the $\MAXV$ function considers $O(|Q|)$ queries ($O(m^2)$ assuming all possible queries) and for each of them finds the variance in $O(1)$ time using the precomputed prefix-sums. Hence, the total running time of the DP algorithm is $O(kn^2|Q|)$. The additional  space we need to run the DP algorithm is $O(n)$ since we can only store the column $A[*,j-1]$ to compute the values in $A[*,j]$.
The pre-computation phase takes $O(n\log n)$ to sort the sampled points, $O(N\log n)$ to construct the prefix sums $X$, and $O(n)$ to create the prefix sums $Z, Y$.

After we find the optimum partition we build a binary balanced search PASS structure where the leaves of the tree are the buckets of the partition. The height of that tree is $O(\log k)$ and for each query we visit $O(\log k)$ nodes.

\remove{
If we need $O(\Delta)$ time to construct the oracle $OPT$, and each oracle query takes $O(Z)$ time, the total running time of our algorithm is $O(\Delta+m^2\cdot k\cdot Z)$.


Next, we show how to construct oracle $OPT$ in $O(m^2\log^4 m)$ time with $O(1)$ query time. Hence, the total running time of our algorithm will be $O(m^2(k+\log^4 m))$.



\paragraph{Oracle}
For each pair $h, i$ that defines a bucket, our goal is to compute $OPT(S[h,i])$.
For each pair of sample points $t_j, t_l$ we create a point in the $2$-dimensional space with coordinates $(j,l)$. Let $B$ be the set of $2$D points, with $|B|=m^2$. We construct a range tree \cite{} $T_B$ on $B$ so that given a query rectangle $\rho$ it returns a set of $O(\log^2 m)$ canonical subsets (rectangles) that contain all points in $\rho\cap B$. The range tree in $2$D is a two level balanced tree. Such a tree can be constructed in $O(m^2\log m)$ and it has $O(m^2\log m)$ size.
For each node $v$ in the second level of the range tree, let $\rho_v$ be the corresponding rectangle and let $B_v$ be the points in $B\cap \rho_v$.
For each point $b\in B$ with coordinates $(j,l)$ we construct a new point with coordinates $b'=(\frac{1}{(l-j+1)^2}\sum_{f=j}^lt_f^2, -\frac{1}{(l-j+1)^2}(\sum_{f=j}^lt_f)^2)$.
All possible sums $\sum_{f=j}^lt_f^2$, or $\sum_{f=j}^lt_f$ can easily be computed by computing prefix-sums in $O(m)$ time. 
Let $B'=\{b'\mid b\in B\}$. Similarly, we define $B_v'=\{b'\mid b\in B_v\}$.
For each node $v$ in the second level of the range tree $T_v$ we construct a halfplane reporting index $T_v$ \cite{} on the $2$D points $B_v'$. $T_v$ can be constructed in $O(|B_V|\log |B_v|)$ and has space $O(|B_V|)$ so in total, all halfplane reporting indexes we build for every node can be constructed in $O(m^2\log^2 m)$ time and have $O(m^2\log m)$ size.
Given a query vector $(x,y)$, $T_v$ can be used to find the point $b'\in B_v'$ with the maximum inner product with vector $(x,y)$ in $O(\log^2 m)$ time.
Using the index we constructed we show describe how we can find $OPT(S[h,i])$. Let $\rho$ be the rectangle defined as $[h,i]\times [h,i]$. Notice that any pair $h',i'$ of sampled points belongs in $\rho$ if and only if $h\leq h'< i$ and $h< i'\leq i$. Let $V$ be the set of $O(\log^2 m)$ canonical subsets of the range tree $T_B$ that partition the points in $B\cap \rho$. Let $v\in V$. We define the vector $u=(i-h+1,1)$ and we run a top-$1$ query in $T_v$ so we return the point with the maximum inner product. Let $b'$ be the point with the maximum inner product among all canonical subsets and let $b=(j,l)$. 
We show that $S[j,l]$ has the largest variance in $S[h,i]$. Given a node $v\in V$ it is sufficient to show that the point $b'\in B_v'$ with the maximum inner product corresponds to a sub-interval with maximum variance. Recall that the query vector is defined as $u=(i-h+1,1)$ and and point $b'$ has coordinates $(\frac{1}{(l-j+1)^2}\sum_{f=j}^lt_f^2, -\frac{1}{(l-j+1)^2}(\sum_{f=j}^lt_f)^2)$. So the inner product is equal to $\frac{i-h+1}{(l-j+1)}\sum_{f=j}^lt_f^2 - \frac{1}{(l-j+1)^2}(\sum_{f=j}^lt_f)^2$ which is equal to the variance in the subset $S[j,l]$. The result of the maximum inner product is multiplied by $\frac{1}{i-h+1}(1-\frac{i-h+1}{N_{i,h}})$ to get the estimated variance of $S[j,l]$ with respect to the bucket $[h,i]$, where $N_{h, i}$ is the total number of tuples (not only sampled) that lie between $t_h$ and $t_i$.
Since there are $O(\log^2 m)$ canonical subsets and for each of them we run a query to find the maximum inner product in $O(\log^2 m)$ time the total query time to compute $OPT(S[h,i])$ is $O(\log^4 m)$.

For each pair of sampled tuples $t_h, t_i$ we run a query in our index and store the value $OPT(S[h,i])$. In total we spend $O(m^2\log^4 m)$ to construct the oracle. For each query the oracle returns the answer in $O(1)$ time.

In total our dynamic programming algorithm runs in $O(m^2(\log^4 m + k))$ time.
}

\mparagraph{Boundaries on any position}
The DP algorithm we presented above finds the optimum partition assuming that the boundaries of the buckets lie on the sampled points. In this paragraph we describe how we can handle the case where the boundaries can be placed anywhere in the domain of attribute $C$.
Assume that we have $N$ tuples in total.
The main idea is to consider $O(\log N)$ possible boundaries between two consecutive sample tuples.
In particular, between two consecutive sampled tuples we consider the tuples that are $2^i$ apart from the sampled tuples. In the DP algorithm, instead of considering $n$ possible locations to place the boundaries we consider $O(n\log N)$ possible locations. In this way the DP procedure will consider a partition where each interval contains the same sampled items as in the optimum  partition and the size of each bucket is within a factor of $2$ of the size of the optimum buckets.
Hence, we can show that the DP algorithm will return a partition with the optimum error for AVG queries (notice that AVG query does not depend on $N_b$ for a bucket $b$), and a partition with error at most a constant factor larger than the error of the optimum partition for SUM and COUNT queries.
We need $O(N\log N)$ pre-processing time to identify the $O(\log N)$ points between the consecutive sampled tuples. The running time of the new DP algorithm is $O(km^2\log^2 (N)|Q|)$.\zs{the problem is when we need this. it sounds like this approach (e.g. when the partition boundaries could lie between sample points) helps on the generalizability of the partition? in this case, we need to say more about the generalizability problem}


\mparagraph{Improving the running time}
In this paragraph we describe how we can improve the running time of our DP algorithm making a mild assumption. For SUM and COUNT queryies we assume that the sample rate for any query interval is roughly the same, i.e., for any interval $\rho$, $\frac{n_\rho}{N_\rho}\approx \alpha$ for $\alpha<1$. We do not need this assumption for AVG queries.
If that holds then we can make the following argument. Let $q$ be a query inside a bucket $b$ and let $b'$ be another bucket such that $b\subseteq b'$, i.e., $b'$ contains $b$.
Then we can show that $V_b(q)\leq V_{b'}(q)$. The exact proof depends on the type of the query. For example for the AVG query, where it holds even without the assumption that $\frac{n_b}{N_b}\approx \alpha$, we have that $S_{b,q}=S_{b',q}$, $n_{b,q}=n_{b',q}$ and $n_b<n_{b'}$. Hence, $V_b(q)=\frac{1}{n_{b,q}^2}\left[\sum_{h\in S_{b,q}}t_h^2 - \frac{\left(\sum_{h\in S_{b,q}}t_h\right)^2}{n_b}\right]\leq \frac{1}{n_{b',q}^2}\left[\sum_{h\in S_{b',q}}t_h^2 - \frac{\left(\sum_{h\in S_{b',q}}t_h\right)^2}{n_{b'}}\right]=V_{b'}(q)$.
Then we can argue that for $h_1\leq h_2$ it holds that $A[h_1,j-1]\leq A[h_2,j-1]$ and $\MAXV([h_1+1,i])\geq \MAXV(h_2+1,i)$. The second inequality holds because of our last observation.
The first inequality holds because we can use the partition of $A[h_2,j-1]$ in the first $h_1$ samples as a valid partition, so $A[h_1,j-1]$ can only be smaller. Because of this property, a ternary search over the values of $h$ can return the value $\hat{h}$ such that $\max\{A[\hat{h},j-1], \MAXV([\hat{h}+1,i])\}$ is minimized. The running time of this DP algorithm is $O(km\log(m)|Q|)$.

\remove{
Assume that $[g,h]$ is an interval in a bucket $[i,j]$. Then let $V_{gh}^{ij}$ is the variance of interval $[g,h]$ with respect to the bucket $[i,j]$. Let $[i',j']$ be a larger bucket with $i'\leq i$ and $j'\geq j$. Intuitively, we would like to argue that $V_{gh}^{ij}\leq V_{gh}^{i'j'}$. If this property holds we can show a faster DP algorithm.

However, there are extreme cases that will happen with relatively small probability where this property does not hold. For example, assume the following instance. Let $b$ be a bucket with $n_b=10$, $N_B=15$ and let $\rho$ be an interval  containing $6$ sampled items with values $1, 1, 1, 0, 0, 0$. Then, we compute $V_\rho^b\approx 0.019$. Now,  assume a larger bucket $b'$ with $n_{b'}=15$ and $N_{b'}=20$ (the difference between bucket $b, b'$ is that $b'$ contains $5$ sampled items more than the bucket $b$). In this case $V_\rho^{b'}\approx 0.016<V_\rho^{b}$, i.e., the variance of interval $\rho$ is larger with respect to the smaller bucket $b$.

We make the following assumption:
For all different possible buckets $[i,j]$ the sample rate is almost the same. For example for any bucket $b_i$ we have $\frac{n_i}{N_i}\approx \alpha$ for a sample rate $\alpha$.
If this is the case then we can show that $V_\rho^{b'}\leq V_\rho^{b}$ for an interval $\rho$ and buckets $b\subseteq b'$. In particular we have $V_\rho^{b}=(1-\alpha)\frac{1}{n_{b,\rho}^2}\sum_{t\in \rho} t^2 - (1-\alpha)\frac{1}{n_{b,\rho}^2}\frac{1}{n_b}(\sum_{t\in \rho} t)^2$. Similarly $V_\rho^{b'}=(1-\alpha)\frac{1}{n_{b',\rho}^2}\sum_{t\in \rho} t^2 - (1-\alpha)\frac{1}{n_{b',\rho}^2}\frac{1}{n_{b'}}(\sum_{t\in \rho} t)^2$. Notice that $n_{b,\rho}=n_{b',\rho}$ while $n_b\leq n_{b'}$. So we conclude that $V_\rho^{b'}\leq V_\rho^{b}$.

If the property above holds then we can make the next argument for the DP algorithm. Recall the recursion 
$A[i,j]=\min_{h<i}\max\{A[h,j-1], MAX(S[h+1,i])\}$. If the sample rate is for all possible buckets roughly $\alpha$ then for $h_1\leq h_2$ we have $A[h_1,j-1]\leq A[h_2,j-1]$ and $MAX(S[h_1+1,i])\geq MAX(S[h_2+1,i])$. By running a ternary search over the values of $h$ we can get the value $\hat{h}$ such that $\max\{A[\hat{h},j-1], MAX(S[\hat{h}+1,i])\}$ is minimized.
}


\mparagraph{Faster approximation algorithm for computing $\MAXV$}

All the algorithms we proposed so far compute the query with the maximum variance in a range $[i, j]$ by considering all possible queries in $[i,j]$. In the worst case the function $\MAXV([i,j])$ can be computed in $O(|Q|)$ time, where $|Q|=O(m^2)$. Hence, the algorithm might not be practical in large datasets. Here, we propose a way to compute an approximation of $\MAXV[i,j]$ more efficiently. We call this function $\AMAXV$.

The high level idea is the following: We divide the $j-i+1$ samples into smaller groups. In order to find the query with the largest variance we consider all possible queries with  respect to the boundaries of the smaller groups. In the end we show that if groups are small enough we can get an approximation of the query with largest variance.

We first start by introducing some useful notation.
Let $\Gamma=\frac{\max_{j}t_j}{\min_{j: t_j>0}t_j}$ be the spread of the values of the non-zero sampled items.
Without changing the result of our algorithm we scale all aggregate values of the sampled items such that $\min_{j: t_j>0}t_j=1$, so it holds that $\Gamma=\max_{j}t_j$.
Notice that for binary values of the tuples $t$ (for example in COUNT queries), $\Gamma=1$.
%Notice that these are reasonable assumptions since each bucket and query should contain sufficient number of sampled points in order to be able to have a reasonable estimation of the variance.

We are ready to describe our new procedure for computing $\AMAXV(\rho)$, for an interval $\rho$.
Let $\eps$ be a parameter such that $\eps\leq \frac{1}{32\Gamma}$.\footnote{The constant $32$ is not important. We can choose a smaller constant making the approximation worse by a constant factor.}
We divide the samples in $\rho$ to $L=\frac{1}{\eps}$ groups such that each group contains at most $\eps n_\rho$ items. Let $G_\rho=g_1,\ldots, g_{L+1}$ be the $L+1$ boundaries of the sampled points. For each pair $g_u, g_v\in G$, if there are more than $\delta n$ sampled points in $[g_u, g_v]$ (i.e., $[g_u,g_v]$ is a valid query) we compute the variance of the query $[g_u, g_v]$. In the end we return the maximum variance over all possible queries defined by $G$.


Using the pre-computed values of $X, Y, Z$ we described above, $\AMAXV$ runs in $O(\frac{1}{\eps^2})$ time.

Next we show that the result returned by our new procedure is close to the variance of the query with the maximum variance in $\rho$.
For simplicity, we assume that $\delta< \frac{1}{32\Gamma}$ and $n\geq \frac{1}{\delta\eps}$, so that each group contains at least one sampled item.
We focus on the case where $n_\rho\geq 2\delta n$. Similarly we can also handle the case where $n_\rho< 2\delta n$ making some assumptions. Alternatively, in practice, we can assume that the maximum variance query in this bucket is $0$ or $n_\rho$ is so small that we can compute the query with the maximum variance in a brute force manner.

We show the approximation factor for the SUM query, and in the end we show how to extend to AVG and COUNT queries.
Let $q$ be the query with the maximum variance in $\rho$. Let $g_l, g_r$ be the boundaries of the groups with the smallest distance such that $q$ lies between $g_l, g_r$.
Let $q'=[g_l,g_r]$. Notice that our approximation algorithm considers query $q'$ since it is defined by the boundary points. Furthermore, $n_{q'}\geq \delta n$ since $q'$ contains $q$. We show that the variance of $q'$ approximates the variance of $q$.

Let $b_l, b_r$ be the groups defined by $[g_l, g_{l+1}]$, and $[g_r,g_{r+1}]$, respectively. Let $b=b_l\cup b_r$. If $g_{l+1}=g_r$ then $b$ is the group defined by $[g_l,g_r]$.
For simplicity we skip the factors $\frac{1}{n_\rho}\cdot\frac{N_\rho^2}{n_\rho^2}$ in the variance $V$ since they are the same for all queries in $\rho$.
We have,
\begin{align*}
V_{q'}&=n_\rho \sum_{h\in q'}t_h^2-(\sum_{h\in q'}t_h)^2\\
&=n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2 + n_\rho \sum_{j\in b\setminus q}t_j^2 - (\sum_{j\in b\setminus q}t_j)^2 - 2\sum_{h\in q}t_h \sum_{j\in b\setminus q}t_j.
\end{align*}
Next, we show our main observation: $V_{q'}\geq \frac{1}{2}\left[n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2\right]$.
\stavros{The next can all be in a lemma showing that argument}

We note that this is equivalent with showing that 
$$A=n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2 + 2\left[n_\rho \sum_{j\in b\setminus q}t_j^2 - (\sum_{j\in b\setminus q}t_j)^2\right] - 4\sum_{h\in q}t_h \sum_{j\in b\setminus q}t_j\geq 0$$
We observe that $n_\rho \sum_{j\in b\setminus q}t_j^2 - (\sum_{j\in b\setminus q}t_j)^2\geq 0$ and $\sum_{j\in b\setminus q}t_j\leq \sum_{j\in b}t_j$. Hence, 
$A\geq n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2 - 4\sum_{h\in q}t_h \sum_{j\in b}t_j$.
It also holds that $\sum_{j\in b}t_j\leq 2\eps n_\rho\Gamma$, and $\sum_{h\in q}t_h\leq \sum_{h\in q}t_h^2$, so
$$A\geq n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2 - 8\eps\Gamma n_\rho \sum_{h\in q}t_h^2.$$

Before we continue we make the following useful observation. For any query $\hat{q}$ in $\rho$, it holds that $n_\rho\sum_{h\in\hat{q}}t_h^2-(\sum_{h\in \hat{q}}t_h)^2 = (n_\rho-1)\sum_{h\in\hat{q}}t_h^2 - 2\sum_{i<j\in \hat{q}}t_it_j = (n_\rho-n_{\rho,\hat{q}})\sum_{h\in\hat{q}}t_h^2+ (n_{\rho,\hat{q}}-1)\sum_{h\in\hat{q}}t_h^2 - 2\sum_{i<j\in \hat{q}}t_it_j = (n_\rho-n_{\rho,\hat{q}})\sum_{h\in\hat{q}}t_h^2 + \sum_{i<j\in \hat{q}}(t_i-t_j)^2$. Hence, notice that if $n_{\rho, \hat{q}}\leq n_\rho/2$, then $n_\rho\sum_{h\in\hat{q}}t_h^2-(\sum_{h\in \hat{q}}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in\hat{q}}t_h^2$.

Now, we continue with the proof of our main argument.
We consider two cases.

%If $n_{\rho,q}\leq n_\rho/2$ then from our observation, 
%$n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in q}t_h^2\geq 8\eps\Gamma n_\rho \sum_{h\in q}t_h^2$. The last inequality holds because $\eps\leq \frac{1}{32\Gamma}$. Hence, we conclude that $A\geq 0$.

%Next, we consider $n_{\rho,q}>n_\rho/2$. We take two more sub-cases.

Let assume that $n_{\rho,q}\geq 2\delta n$. In this case, let $q_l, q_r$ be two queries with $n_{\rho, q_l}=n_{\rho,q_r}=n_{\rho,q}/2$ such that $q_l$ has its left boundary on the left boundary of $q$ and $q_r$ has its right boundary on the right boundary of $q$. Notice that $q=q_l\cup q_r$ and $q_l\cap q_r=\emptyset$. Without loss of generality assume that $\sum_{h\in q_l}t_h^2\geq \sum_{h\in q_r}t_h^2$, so $\sum_{h\in q_l}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$. We also observe that $n_{\rho,q_l}\leq n_\rho/2$.
Notice that $q$ is the query with the largest variance in $\rho$ and $q_l$ is a valid query since $n_{\rho,q_l}=n_{\rho,q}/2\geq \delta n$. Hence, $V_q\geq V_{q_l} \Leftrightarrow n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2\geq n_\rho \sum_{h\in q_l}t_h^2-(\sum_{h\in q_l}t_h)^2 \geq \frac{n_\rho}{2}\sum_{h\in q_l}t_h^2\geq \frac{n_\rho}{4}\sum_{h\in q}t_h^2\geq 8\eps\Gamma n_\rho \sum_{h\in q}t_h^2$. The last inequality holds because $\eps\leq \frac{1}{32\Gamma}$. Hence, we conclude that $A\geq 0$.

The last case to consider is when $n_{\rho,q}<2\delta n$. This is similar to the previous case. Let $q_l, q_r$ be queries with $n_{\rho, q_l}=n_{\rho,q_r}=\delta n$ where the left boundary of $q_l$ is the left boundary of $q$ and the right boundary of $q_r$ is the right boundary of $q$. In this case notice that $q_l\cap q_r\neq \emptyset$. Without loss of generality we assume that $\sum_{h\in q_l}t_h^2\geq \sum_{h\in q_r}t_h^2$, so $\sum_{h\in q_l}t_h^2\geq \frac{1}{2}\sum_{h\in q}t_h^2$. We also observe that $n_{\rho,q_l}\leq n_\rho/2$ since $n_{\rho,q_l}=\delta n$ and $n_\rho\geq 2\delta n$.
Notice that $q$ is the query with the largest variance in $\rho$ and $q_l$ is a valid query since $n_{\rho,q_l}=\delta n$. Hence, $V_q\geq V_{q_l} \Leftrightarrow n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2\geq n_\rho \sum_{h\in q_l}t_h^2-(\sum_{h\in q_l}t_h)^2\geq \frac{n_\rho}{2}\sum_{h\in q_l}t_h^2\geq \frac{n_\rho}{4}\sum_{h\in q}t_h^2\geq 8\eps\Gamma n_\rho \sum_{h\in q}t_h^2$. The last inequality holds because $\eps\leq \frac{1}{32\Gamma}$. Hence, we conclude that $A\geq 0$.

Overall, we showed that $V_{q'}\geq \frac{1}{2}V_q$.
The same holds for COUNT queries.
The running time is bounded by $O(\Gamma^2)$ (notice that for SUM or COUNT queries there is no advantage choosing $\eps<\frac{1}{32\Gamma}$).
For AVG queries, if we repeat the analysis we get $V_{q'}\geq \frac{1}{n_{\rho,q'}}\frac{1}{2}[n_\rho \sum_{h\in q}t_h^2-(\sum_{h\in q}t_h)^2]$, so $V_{q'}\geq \frac{n_{\rho,q}^2}{n_{\rho,q'}^2}\frac{1}{2}V_q\geq \frac{n_{\rho,q}^2}{(n_{\rho,q}+2\eps n_\rho)^2}\frac{1}{2}V_q$. Using the arguments of the proof above, we can show that the AVG query with the maximum variance in $\rho$ contains at most $2\delta n$ elements. In the worst case $\frac{n_{\rho,q}^2}{(n_{\rho,q}+2\eps n_\rho)^2}\geq \frac{(\delta n)^2}{(\delta n+2\eps n)^2}=\left(\frac{\delta}{\delta+2\eps}\right)^2$, so $V_{q'}\geq \frac{1}{2}\left(\frac{\delta}{\delta+2\eps}\right)^2V_q$, for AVG queries. The running time is $O(\frac{1}{\eps^2})$.
If we set $\eps=\delta$ then we can get $\frac{1}{18}$-approximation in $O(\delta^2)$ time.

%We can also have the same conclusion for the special case where $n_\rho<2\delta n$ assuming that the query $q$ with the maximum variance has $n_{\rho,q}<\alpha n_\rho$ for a constant $\alpha$.


By replacing $\MAXV$ with $\AMAXV$ in the DP algorithm we get the recursion
$A[i,j]=\min_{h<i}\max\{A[h,j-1], \AMAXV([h+1,i])\}$. The new DP algorithm runs in $O(km\log(m)\Gamma^2)$ time for SUM and COUNT queries.
By skipping some low level details we can show that \stavros{If the intuition is not very clear , if needed and we have space, I can add the full proof (how an $\frac{1}{\alpha}$-approx for $\MAXV$ gives an $\alpha$-approx for the our problem using the DP)}
%for a cell $A[i,j]$, the approximated value $V$ found by the DP algorithm, using $\AMAXV$, satisfies $\frac{1}{\alpha}V'\leq V\leq V^*$, where $V^*$ is the variance of the optimum partition in $A[i,j]$, $V'$ is the real variance of the partition found by the DP algorithm, and $\alpha$ is the approximation ratio of finding the query with the maximum variance in an interval $[h,i]$. \stavros{I can add the full proof if is needed and we have space.} Hence, we can show that
our new algorithm finds a partition where the maximum variance query is at most $\sqrt{2}\cdot\sqrt{2}=2$ times the maximum variance query of the optimum partition for SUM and COUNT queries.
For AVG queries the DP runs in $O(km\log(m)\frac{1}{\eps^2})$ time
and finds a partition where the maximum variance query is at most $\sqrt{2}\frac{\delta}{\delta+2\eps}$ times the maximum variance query of the optimum partition.




\subsection{Partition in any dimension}
\label{sec:kd-tree}

While the DP algorithm gives an optimum partition for Problem 1 given a sample set $S$ it is not easy to extend it to higher dimensions. In this section we propose a method to find an optimum partition in any dimensions $d\geq 1$ efficiently. For simplicity, we assume that $d$ is a constant.

One possible solution is to use the method proposed by the AQP++ method~\cite{}. The idea is to estimate the error in each dimension and identify suitable $k_1, k_2, \ldots, k_d$ such that $\prod_{i=1}^dk_i\leq k$.
Then they use their Hill Climbing algorithm to find a partition in the $i$-th dimension using $k_i$ buckets.
In our case, we can use our DP algorithm to find an optimum or near optimum partition of $k_i$ buckets in each dimension $i$.
In the end we get a (non-uniform) grid with $k$ boxes in $\Re^d$ and we build a balanced tree with $k$ leaf nodes where each node corresponds to a box in the partition.

While the method above is practical and give some reasonable partitions in real data~\cite{}, it does not have a theoretical guarantee. Here, we propose a partition in $\Re^d$ which is near-optimum assuming following a specific geometric structure.

Assume that we are able to find the best partition of $k$ hyper-rectangles \zs{or high-d ``rectangles''} \stavros{Yes, we can agree to a term and use it everywhere. In geometric papers i have seen rectangles (not only for 2 but for any dimension), hyperrectangle, or just box, which is my favorite.} that minimizes the maximum variance of a query. In our case we would like to build a tree structure on the given optimum partition so that given a query we can bound the number of nodes of the tree we have to visit. However, if we get an optimum arbitrary partition of $k$ rectangles it is not always clear how to construct a tree with small height and small query time (for example if the partition is not a grid). \zs{i'm not sure whether this is the best argument. we can talk about this}In this section we aim to find the optimum partition in a constrained domain. More specifically, we focus on finding the best partition of $k$ rectangles, where the rectangles are chosen from a balanced kd-tree of the sample set $S$.

A balanced kd-tree is a tree structure that partitions the data in $\Re^d$. Consider a set of $m$ points $P$ in $\Re^d$. Each node $v$ of the tree is associated with a rectangle $\square_v$. Let $P_v=P\cap \square_v$ and  $m_v=|P_v|$. A node $v$ is a leaf if its associated rectangle contains one point of $P$, $m_v=1$. Otherwise a node $u$ has $2^d$ children constructed as follows. We get the median of the first coordinate of the points in $P_u$ and we divide the points into two equal-size point sets, where the first (second) point set contains the points in $P_u$ with first coordinate less (larger) than the median. We continue doing the same recursively for the rest of the dimensions. In the end we get a partition of $P_u$ into $2^d$ rectangles where each of them contains $O(\frac{n_u}{2^d})$ points of $P_u$.
All the rectangles created in the kd-tree are called canonical rectangles. 
The height of the tree is $O(\log m)$.  A balanced kd-tree can be constructed in $O(m\log m)$ time, has $O(m)$ space and given a query rectangle $\rho$ it finds a set of $O(m^{1-1/d})$ canonical rectangles that partition $\rho$ in $O(m^{1-1/d})$ time.

We study the following problem. Let $T$ be the balanced kd-tree constructed on our sampled items $S$.
The goal is to find an optimum partition of $S$ into $k$ canonical rectangles of $T$.
For simplicity, we assume that $k=t\cdot 2^d$.

We start by doing some pre-computation. We construct $T$, the balanced kd-tree constructed on our sampled items $S$. For each node $u$ in $T$ we store $n_u=|S\cap \square_u|$.
Furthermore, we store $N_u$, the number of items in the database that lie in $\square_u$. We can find the values $N_u$ by searching for each item $p$ in the database the leaf $v$ such that $p\in \square_v$. Then we increase all values $N_u$ for $u$ in the path from the root to $v$. Finally, for each node $u$ in $T$ we keep $\sum_{t\in S\cap \square_u} t$ and $\sum_{t\in S\cap \square_u} t^2$.

Let $T'$ be the tree that we are going to build. At the beginning, $T'$ contains only the root of $T$. While the number of leaf nodes is less than $k$, we repeat the following.
For each leaf node $v$, that was created in the previous iteration of the algorithm, we run the function $\MAXV(v)$.
The function $\MAXV$ is similar to the $\MAXV$ function in the DP algorithm. The only difference is that it uses the pre-computed values in $T$ to find the query with the largest variance in a node. We skip the low level details since they are similar to the DP case. Let $u$ be the leaf of $T'$ that contains the query with the largest variance and let $C(u)$ be the children of $u$ in $T$. We add $C(u)$ as the children of $u$ in $T'$.

The running time of the pre-computation is $O(m\log m)$ to construct $T$ and to find the $n_u$ values. In order to find the $N_u$ values we need $O(N\log m)$ time since the height of $T$ is $O(\log m)$. After the precomputation, the algorithm runs in $O(km^{1-1/d}|Q|)$ time\footnote{If we use a range tree~\cite{} to find the number of sampled items in a rectangle $\rho$ then the running time can be improved to $O(k|Q|\polylog(m))$ time.}.

Next we show that the partition of $T'$ is optimum with respect to tree $T$.


\begin{lemma}
The tree $T'$ returned by our algorithm has the optimum partition, with respect to $T$.
\end{lemma}
\begin{proof}
First, notice that Lemma~\ref{lem:Obs} holds for any dimension $d\geq 1$. Hence, it is always sufficient to check the queries with at least $\delta n$ sampled items that lie completely inside a rectangle $\square_u$ for a leaf node $u$ of $T'$ to find the query with the maximum variance.
Second, as we highlighted in the faster implementation of the DP algorithm, if $u$ is an ancestor of $v$ in $T$, and $q$ is a valid query in $v$ then for the AVG query $V(q,v)\leq V(q,u)$, where $V(q,v)$ is the variance of query $q$ in bucket $v$. If we assume that the sample rate in each node of the tree is roughly equal ,the same holds for SUM and COUNT queries. Hence, the overall maximum variance of $T'$ is always non-increasing as we run more iterations.

Let $T^*$ be the optimum tree with $k$ leaf nodes with error $V(T^*)$. If $T'$ is identical to $T^*$ then $T'$ is optimum. Next we consider the case where $T'$ is not identical to $T$. Assume that $V(T^*)<V(T')$. Since $T'$ is not identical to $T^*$, there will always be a leaf node $u$ of $T^*$, where $u$ belongs in $T'$ and $u$ is not a leaf node in $T'$. In other words, $u$ is a leaf node in $T^*$, however in one of the iterations of our algorithm we found that $u$ had the query with the largest variance and we added its children from $T$. Let $V(u)$ be the error of the query with the maximum variance in node $u$. Since, the children of $u$ were added in $T'$ we have that $V(T')\leq V(u)$. However, $u$ is a leaf node of $T^*$, so $V(T^*)\geq V(u)$, which is a contradiction. We conclude that $T'$ is a tree with minimum variance.
\end{proof}

The same construction works for the estimation of any query AVG, SUM, COUNT.
The tree $T'$ we constructed is optimum with respect to queries that lie completely inside the cells of the kd-tree. Hence, we get an optimum partition with respect to $T$ for AVG queries and a $\sqrt{k}$-approximation for SUM and COUNT queries.


Even though this algorithm can be used for any dimension $d$ it can also be used for $d=1$. In that case we would get a $O(k|Q|)$ algorithm for constructing a partition after the pre-computation. That improves the running time of the DP algorithm, however the DP guarantees a near optimum partition, while $T'$ guarantees a near optimum partition only with respect to the kd-tree $T$ with $k$ leaf nodes.

Similarly to the $1$-dimensional case we can run the $\AMAXV$ procedure to get an approximation of the maximum variance query in a rectangle $\rho$. By extending the algorithm for $\AMAXV$ from $1$D to any dimension $d$ for SUM and COUNT queries, we can get a $O(\frac{1}{\Gamma})$-approximation of the maximum variance query in a rectangle. For AVG queries we can get $O(\Gamma\delta^2)$-approximation.
The running time of the $\AMAXV$ algorithm in $d$-dimensions is $O(\Gamma^{2d})$.
Using $\AMAXV$ in the construction of the kd-tree we get $O(\sqrt{k\Gamma})$-approximation of the optimum kd-tree partition in $O(km^{1-1/d}\Gamma^{2d})$ time for SUM and COUNT queries. In the same time we can get $O(\frac{1}{\sqrt{\Gamma}\delta})$ approximation of the optimum kd-tree partition for AVG queries.

\mparagraph{Extensions}

Even though, our partition is optimum with respect to a kd-tree partition, the height of the tree we construct in the worst case can be $O(\min\{k, \log m\})$. For example, assume that the algorithm always splits a node at height $i$ in the $i+1$ iteration. In this case, $T'$ will have $O(k)$ height, so when a query comes it might need to visit $O(k)$ leaf nodes of the tree. If we want to guarantee faster query time in the worst case we need to guarantee that the leaf nodes in tree $T'$ do not have a big depth difference. Assuming a parameter $\tau$, in practice, each time that we decide to further split a node $u$ we check whether there is a leaf node $v\in T'$ such that $depth(u)-depth(v)>\tau$. If this is the case, we also split the node $v$. After we make sure that the maximum difference in depth is $\tau$, we continue by splitting the node that contains the maximum variance query.



% \subsection{Partitioning Algorithm}

% Given the discussion of optimization problem above, and the way we combine sampling and PA to solve a query: 

% \[
% Sol(Q) = PA(Q') + \sum_{q_i \in \Delta Q, \cup q_i = \Delta Q, \cap q_i = \emptyset }{Sampling(q_i)}
% \]

% The goal of minimizing the average/maximum variance is equivalent to minimizing the average/maximum size of $\Delta Q$ for each query in the workload.

% If the workload is given without a storage constraint for partitioning, we can build a perfect partition $P^*$ with which every query in the workload can be perfectly aligned on the edge of one of more partitions thus introduce a 0 error, i.e. $\Delta Q = \emptyset$. Now to satisfy a constraint $k$ over the size of the partition. We can use the following bottom-up greedy algorithm. Given a partition $P$, We use $\Delta(q, P)$ to denote the area of the redundant rectangles when solving a query $q$ with partition $P$. We define a cost function $cost(p_i, p_j)$ to be the cost of merging neighboring partition $p_i$ and $p_j$ from $P$: 

% 1) To minimize the max variance, the cost function is the largest $\Delta Q$ introduced by the merge among all the queries, i.e.:
% \[
% cost(p_i, p_j) = \max_{q\in Q}{(\Delta(q, merge(p_i,p_j)))}
% \]


% 2) To minimize the average variance, the cost function is the sum of $\Delta Q$ introduced by the merge among all the queries, i.e.:
% \[
% cost (p_i, p_j) = \sum_{q\in Q}{(\Delta(q,  merge(p_i,p_j)))}
% \]

% We use a MinHeap $H$ to facilitate the process.

% \begin{algorithm}[h]
% \SetAlgoLined 
%  Input: partition size $k$, a perfect Partition $P^*$ for workload $Q$\;
%  Output: a partitioning $\mathcal{P}$ of size $k$ \;
%  Initialization: MinHeap $H$\;
%  \For{$p_i$, $p_j$ $\in$ $P^*$}{
%     \If{IsNeighbor($p_i, p_j$)}{
%         H.push($cost(p_i, p_j)$)
%     }
%  }
 
%  \While{|H| > k}{
%   $p_i$, $p_{i+1}$ = H.pop()\;
%   let $p_i$ = merge($p_i$, $p_{i+1}$)\;
%   re-calculate $cost(p_{i-1}, p_i), cost(p_{i}, p_{i+2})$\;
%   replace $cost(p_{i-1}, p_i), cost(p_{i}, p_{i+2})$ in $H$\;
%  }
%  \caption{Bottom-up Partitioning}
% \end{algorithm}


% \subsection{Cross Layer Estimation with Stratified Sampling}
% \label{sec:crosslayer}
% As described in Section \ref{sec:sys-design}, a data chunk assigned to a layer of the PA tree form a strata which we can use for stratified sampling. And the strata in the layer $h+1$ are more fine grain than the the ones in layer $h$. Therefore, if we traverse deeper and spend more budget we can always get a better answer in layer $h+1$ than in layer $h$. 

% Naively, we could solve a query iteratively: we solve the query with strata of the current layer as we traverse until we run out of budget or meet the SLA.

% However, if we only use the result derived in the current layer, the budget we spent from the first layer to the previous layer would be wasted. We could somehow try to merge or combine results derived from two or more different layers. And this is done by calculating a variance weighted arithmetic mean. 

% We first calculate the query result $x_h$ for layer $h$ and its variance $\sigma_h^2$. We assign a weight $\omega_h = \frac{1}{\sigma_h^2}$ which is the reciprocal of its variance and the variance weighted arithmetic mean that combines all layers is given by:

% \[
% \overline{x} = \frac{\sum_{i=1}^h{(x_i\sigma_i^{-2})}}{\sum_{i=1}^h{\sigma_i^{-2}}}
% \]

% With a minimized variance:
% % https://en.wikipedia.org/wiki/Inverse-variance_weighting
% %https://en.wikipedia.org/wiki/Weighted_arithmetic_mean#Variance_weights
% \[
% \sigma_{\overline{x}}^2 = \frac{1}{\sum_{i=1}^{h}\sigma_i^{-2}}
% \]

% \subsubsection{Preliminary Results}

% Figure \ref{fig:clvw} is a preliminary result comparing uniform sampling (US), stratified sampling (ST) and cross layer variance weighted (CLVW) stratified sampling on 1000 random COUNT, SUM and AVG queries. For stratified sampling we construct a tree of different depth and use the strata in the leaf layer to solve the query then scale the result up for the entire dataset. For CLVW, we calculate a result on each layer with $SampleSize=TotalSampleSize$ then compute a variance weighted mean cross different layers. For CLVW-Split, we calculate a result on each layer with $SampleSize=\frac{TotalSampleSize}{TreeDepth}$ then compute a variance weighted mean cross different layers.   PA tree use a equal width (range) partitioning with a fan-out of 4. All results are computed with samples, the PA tree defines the strata but summaries are not used for computation.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=1\linewidth]{exp-figures/clvw.png}
%   \caption{US vs. ST-Leaf of different tree depth vs. Cross Layer Variance Weighted stratified sampling.}
%   \label{fig:clvw}
% \end{figure}


% \subsection{Cross Layer Estimation with PA and Stratified Sampling}
% We can adapt AQP++ approach. Use aforementioned stratified sampling approach to estimate delta then combine with PA results.

% \subsection{How to Meet a SLA}
% \label{sec:sla}
% If the SLA is defined in terms of confidence, high levelly, maybe we can calculate the sample size required by the confidence interval then use that information to generate an efficient query plan? \xl{to think more}



\iffalse
\remove{
We start by introducing some useful notation.
Let $q\in Q$ be a query in $Q$ and $P=\{P_1, \ldots, P_k\}$ be a partition of the sample set $S$ over the attribute $C$, where $P_i$ is the $i$-th bucket in partition $P$. Query $q$ can partially intersect at most two strata, $P_{j_1}, P_{j_2}$ in $P$. Let $S$ be the sample set of size $m$, $S_i$ be the samples from stratum $P_i$, $N_i$ be the size of stratum $P_i$, $N_{i,q}$ be the number of tuples in $P_i$ satisfying the query $q$, $n_i=|S_i|$ be the sample size of stratum $P_i$, $n_{i,q}$ number of samples in $P_i$ satisfying $q$.

We define $|Q|$ as the number of different queries with respect to the sample set $S$. For example if two queries $q_1,q_2\in Q$ contain the same set of sampled points we count them as one query in $|Q|$. If $Q$ is the set of all possible queries in $R^1$ then $|Q|=O(m^2)$. Generally, if $Q$ is the set of all possible queries in $R^d$ then $|Q|=m^d$.

Let $Pr_q(t)$ be a function which is $1$ if tuple $t$ belongs in $q$, and $0$ otherwise. Let $\phi(t,q)=Pr_q(t)\frac{n_i}{n_{i,q}}t$, and $S_{i\phi}=\{\phi(t,q)\mid t\in S_i\}$.
The mean of $S_{i\phi}$ is found by $E[S_{i\phi}]=\frac{1}{n_{i,q}}\sum_{j=1}^{n_i} Pr(t_{ij})t_{ij}$, where $t_{ij}$ is the value of attribute $A$ of the $j$-th sample in stratum $P_i$.
The variance of $S_{i\phi}$ is defined as $\sigma_{i\phi}^2=\frac{1}{n_i}\sum_{j=1}^{n_i} (\phi(t_{ij}, q)-E[S_{i\phi}])^2= \frac{1}{n_i}\sum_{j=1}^{n_i}\phi(t_{ij}, q)^2 - E[S_{i\phi}]^2=
\frac{1}{n_i}\sum_{j=1}^{n_i} (Pr_q(t_{ij})\frac{n_i}{n_{i,q}}t_{ij})^2 - (\frac{1}{n_{i,q}}\sum_{j=1}^{n_i} Pr(t_{ij})t_{ij})^2$.
The estimate variance of bucket $P_i$ with respect to the query $q$ is defined as $V(i,q)=\frac{1}{n_i}(1-\frac{n_i}{N_i})\sigma_{i\phi}^2$.

If $q$ partially intersects $P_i, P_j$ and fully covers $P_{i+1},\ldots, P_{j-1}$ then we define $error(q,P)=\frac{1}{(\sum_{i\leq h\leq j}N_{j})^2}(N_{i}^2V(i,q)+N_{j}^2V(j,q))$. (If $q$ partially intersects only $P_i$ then $N_{j,q}=0$.)
Given a sample set $S$, recall that Problem 1 is defined as $arg\min_P\max_{q\in Q} error(q,P)$.
}
\fi

==> paqp.tex <==
\section{Partial-Aggregate Approximate Query Processing}

\subsection{Problem Statement}

\subsection{Basic Query Processing}

\subsection{Calculating Error Bounds}

\subsection{Discussion and Extensions}


==> partitioning.tex <==
\section{Optimal Partitioning Problem}

\subsection{Problem Definition}
Suppose we have a query workload $Q$ contains aggregate queries of the form:
\begin{lstlisting}
SELECT agg(attr)
FROM R1,...,RN
WHERE P1 and P2 and ... and PK
GROUP BY ....
\end{lstlisting}

In reality, queries in the workload can have multiple duplication therefore different frequency but for now we assume the queries in the workload are unique. To generate a PA set that can answer the queries in a optimal way, we need to carefully design the partitioning of the dataset from which we extract the set of PAs. The partitioning problem can be formalized as the following optimization problem.

Let $aggr(a, p)$ be the partial aggregation of partition $p$ over attribute $a$, e.g., for SUM query, $aggr(a,p)$ is the summation over attribute $a$ of the tuples in the partition.

Let $\mathcal{P} = \{p_1, p_2, ..., p_n\}$ be a partitioning over the dataset, for a query $q \in Q$, let $\mathcal{I}(q, p)$ be 1 if partition $p$ is relevant to query $q$ and 0 otherwise. Take a $\mathbf{SUM(a)}$ query as an example, the cost function of using partitioning $\mathcal{P}$ to answer a query is:

\[
C(q, \mathcal{P}) = \sum_{p \in \mathcal{P}}{\mathcal{I}(q,p)aggr(a, p)}
\]
I.e., for a SUM query, the cost of a partitioning to a query is simply the summation of the partial aggregates on each relevant partitions.

And the cost of solving a workload $Q$ with partitioning $\mathcal{P}$ is:

\[
\mathbb{C}(Q, \mathcal{P}) = \sum_{q\in Q}C(q, \mathcal{P})
\]

The optimal partitioning $\mathcal{P}$ is the one that can minimize the cost and subject to the constraint on the size of partitioning $\mathcal{S}$:

\[
\mathbf{argmin}_{\mathcal{P}} \mathbb{C}(Q, \mathcal{P})  
\]
\[
\text{subject to: } ~ |\mathcal{P}| \leq \mathcal{S}
\]

Furthermore, a query contains a conjunction of predicates over $d$ dimensions: 
$\Pi = \{\pi_1 \wedge \pi_2, ... \wedge \pi_d\}$. Each partition is a tuple of such a conjunction and one or more partial aggregates: $p=\{\Pi, aggr(a_1), aggr(a_2), ...\}$. Each predicate defines a range that is specified by an upper and a lower boundary $\pi = \{l, u\}$. We denote the length of such a range by $|\pi|$.

We can now define an equivalent problem to the above optimization problem to guide the actual partitioning. 
\[
Cost(q, \mathcal{P})  = \sum_{p \in \mathcal{P}}{\mathcal{I}(q,p)(\prod_{i\in D}|\pi_i|})
\]

We want to minimize the area of the relevant hyper-rectangles to a query and the partitioning that defines the hyper-rectangles also subject to the storage constraint.

\[
\mathbf{argmin}_{\mathcal{P}} \sum_{q\in Q}Cost(q, \mathcal{P})  
\]
\[
\text{subject to: } ~ |\mathcal{P}| \leq \mathcal{S}
\]

\subsection{Partitioning Problem}

Given the storage constraint $\mathcal{S}$, building a set of PAs that can answer the workload optimally is equivalent to merging the queries in workload into $k$ clusters that can fit into the storage. 

The merge operation yields a PA for each cluster, and merge operation can be defined as a general primitive, for example: 
1) it can be a simple 'OR' operation that combines the results from queries in the same cluster, such a PA can answer the queries in the cluster optimally but might not handle other queries well;
2) it can also be a bounding box that covers all queries in the cluster, such a PA has a better generalizability because it can answer queries that fall into the bounding box.

In this section, we treat the partitioning problem as a clustering problem (NP-hard, $k^N$ ways of clustering) and discuss a variation of the classic $K-means$ algorithm that can be used to solve the problem. 

Like the conventional clustering problem, each element to be clustered in our problem could have multiple dimensions. Unlike the conventional clustering problem, in our problem, the conventional metric of minimizing the Euclidean distance is not the metric to be optimized..

Consider the example shown in Figure \ref{rect-merge}, if we were to cluster the three queries represented by the three blue rectangles into 2 clusters so that the Euclidean distance within each cluster is minimal, we would put A and B in the first and C in the second cluster.
However, if we merge A and B, we will generate a bounding box showing in the gray area. This result is obviously worse than putting B and C in the same cluster and A in another which yields a bounding box of the yellow area. This is because our goal is to minimize the error caused by the merge operation, i.e. the redundant area, hence we introduce the following variation of the $K-means$ algorithm that merge $N$ queries in to $k$ clusters:

\begin{figure}
    \includegraphics[width=1\linewidth]{figures/rect-merge.png}
    \caption{Clustering three queries of 2-d predicates.}
    \label{rect-merge}
\end{figure}

Initialization:
    Randomly assign each query an unique integer ID between 0 and $N$, and a cluster label between 0 and $k$;

Step 1: update

    calculate the bounding boxes that covers all rectangles of the same cluster label.

Step 2: assign

    For each rectangle $r_i$, calculate the error when merge each cluster $c_j$ represented by a bounding box, let $MA_{ij}$ be the area of new the bounding box after merge $r_i$ and $c_j$:
\[
    Error = MA_{ij} - Area(r_i) - \sum_{r\in c_j}{Area(r)}
\]

    Assign each rectangle to the cluster with the minimal error.
    
Convergence of the algorithm:


The algorithm stops when the assignment does not change or when the error of new assignment is not better than last iteration. We break tie deterministically by favoring the cluster with the minimum query id. The algorithm does not guarantee to find a global optimum.


==> pc-partition.tex <==
\xl{This is obsolete.}

%connection to data skipping
Note that above formulation of our partitioning problem share some commonalities with the partitioning problem defined in data skipping literature, e.g. \cite{sun2014fine, Shanbhag2017partitioning} \xl{more ref here later}, for example, given a partitioning and a query, both problems have to determine the relevance of a partition to a query. But there is a nuance in the objective functions, in the data skipping problem, we want to partition the dataset in a way to maximize the number of tuples that can be safely skipped, and the query results are always accurate because we only skip irrelevant tuples and the queries are answered by using a super set of relevant tuples. 

%connection to clustering
However, in the PC problem, our goal is to trade accuracy with a decreased cost, the queries are answered by PCs directly without involving the actual tuples in the dataset. Therefore, our objective in the PC partitioning problem is to minimize the inaccuracy that is introduced by partitioning, i.e. the difference between the ground truth and the estimation generated by PC. 

In a sense, both problems aim to isolate the relevant and irrelevant tuples in an optimal way, but due to a different objective the solution might be different. Consider the following example with a table that contains attributes $\mathbf{a}$ and $\mathbf{b}$:

\begin{table}[h]
\begin{tabular}{@{}lllllll@{}}
\textbf{a} & 1 & 2 & 3 & 4 & 5 & 6 \\ \midrule
\textbf{b} & 2 & 4 & 1 & 1 & 1 & 7
\end{tabular}
\end{table}
And a simple query with a ground truth of 7: 
\begin{lstlisting}
SELECT SUM(b) FROM table 
WHERE a >= 2 and a <= 5
\end{lstlisting}

For data skipping, there are two tuples, i.e. (1, 2) and (6, 7) can be skipped so the following partition with $k = 3$ is optimal:
\begin{table}[h]
\begin{tabular}{@{}ll|llll|l@{}}
\textbf{a} & 1 & 2 & 3 & 4 & 5 & 6 \\ \midrule
\textbf{b} & 2 & 4 & 1 & 1 & 1 & 7
\end{tabular}
\end{table}

We consider a simplified form of PC:
\[
\{Predicate, Max(a), Cardinality\}
\]and above partitioning yields a PC set of three PCs: 

$pc_1 = \{[1,1], 2, 1\}$,  $pc_2 = \{[2,5], 4, 4\}$,  $pc_3 = \{[6,6], 7, 1\}$,

the answer to the query is 16, with a cost 16 - 7 = 9. 

However, we can easily verify the following partition is optimal for PC partitioning:

\begin{table}[h]
\begin{tabular}{@{}lll|lll|l@{}}
\textbf{a} & 1 & 2 & 3 & 4 & 5 & 6 \\ \midrule
\textbf{b} & 2 & 4 & 1 & 1 & 1 & 7
\end{tabular}
\end{table}

This partition also yields a PC set of three PCs: 

$pc_1 = \{[1,2], 4, 2\}$,  $pc_2 = \{[3,5], 1, 3\}$,  $pc_3 = \{[6,6], 7, 1\}$,

and the answer to the query is 11 with a cost of 11 - 7 = 4.

%connection to hierarchical partitioning, i.e. k-d tree, heterogeneous tree

%connection to hierarchical clustering


\subsection{Solve the Partitioning Problem}

Intuitively, without a prior of the workload, the partitioning goal of minimizing the overall cost (i.e. the difference between the PC estimation and the ground truth) is equivalent to minimizing the variance of the values of the aggregate attribute of the tuples in each partition. 

Let $\mathbf{d(a, p)}$ be the sum of square of partition $\mathbf{p}$ on attribute $\mathbf{a}$, i.e.,
\[
d(a, p) = \sum_{t\in p}(Attr(a, t) - Mean(a, p))^2 
\]
where $\mathbf{mean(a, p)}$ is the mean value of attribute $\mathbf{a}$ in partition $\mathbf{p}$.
The Ward's minimum variance method \cite{ward1963hierarchical} which is widely used for clustering defines the following objective function that measures how much the sum of squares increases when we merge two partitions $p1,~p2$:
\[
\triangle(p_1, p_2) = d(a, p1\cup p2) - d(a, p1) - d(a, p2)
\]
With Ward's method, we can use the following bottom-up greedy algorithm with a complexity of $\mathbf{O(n)}$ for partitioning:

\begin{algorithm}[h]
\SetAlgoLined 
 Input: partition size $k$, attribute $a$, a dataset $D$\;
 Output: a partitioning $\mathcal{P}$ of size $k$ on attribute $a$\;
 Initialization: MinHeap H\;
 \For{t_i, t_j \in D}{
    \If{IsNeighbor(t_i, t_j)}{
        H.push($\triangle(p_i, p_j)$)
    }
 }\\
 
 \While{|H| > k}{
  $p_i$, $p_{i+1}$ = H.pop()\;
  let $p_i$ = merge($p_i$, $p_{i+1}$)\;
  re-calculate $\triangle(p_{i-1}, p_i), \triangle(p_{i}, p_{i+2})$\;
  replace $\triangle(p_{i-1}, p_i), \triangle(p_{i}, p_{i+2})$ in $\mathcal{H}$\;
 }
 \caption{\\Bottom-up partitioning with Ward's method}
\end{algorithm}

TODO: think more about DP?


OBSOLETE: exact partitioning 

\subsection{Partitioning}

Now, we can introduce the partitioning algorithm which is based on an intuitive idea: we want the boundaries of predicates land exactly on the boundaries of partitions, which means for each query, there is a subset of partitions that cover the predicates of a query exactly, i.e., there is no extra or redundant area. To achieve that, we can split each dimension into disjoint chunks so that the lower bound of each query predicate coincides with a lower bound of the chunk and vice versa for the upper bound.

\textbf{Algorithm 1}: partition a dimension

Let $B$ be the set of unique predicate boundaries collected from a workload of queries: $B = \{b_1, b_2,..., b_m\}$ that are sorted in a ascending order;

Step 1: for each boundary $b$ we assign an $IsLower$ flag if the boundary is a lower boundary of a predicate and an $IsUpper$ if it is upper boundary of a predicate. 

Step 2: we scan the set of annotated boundaries in ascending order and create an augmented list $L'$ of boundaries in Step 3.

Step 3: 
For each boundary $b$:

3.1. if $IsLower$ and $IsUpper$ are both true, we insert $b-1, b, b, b+1$ into $L'$;

3.2. else if only $IsLower$ is true, we insert $b-1, b$ into $L'$;

3.3. else if only $IsUpper$ is true, we insert $b, b+1$ into $L'$;


Step 4: make sure each element in $L'$ occurs no more than twice.

Step 5: scan $L'$ again and for every 2 adjacent elements $b_i, b_{i+1}$, add a partition $[b_j, b_{j+1}]$ for dimension $i$ to list $P_i$.

The algorithm returns a $P_i$ which is a list of partitions for a dimension $i$, the time  complexity is O(n) to the number of queries.


\textbf{Algorithm 2}: partition a dataset of $D$ dimensions

Step1: generate a partition $P_i$ for each dimension i; 

Step2: generate a Cartesian Product over all $P_i$, this will generate a list of partitions for the entire dataset, each partition contains $D$ predicates that defines a hyper-rectangle. The partition is optimal to the workload.

The size of the partition is exponential to the number of dimensions.

The partition can be generated by taking one pass of data. 

What if the memory is not enough to hold?

\textbf{Algorithm 3}: enforce the storage constrain

We merge the adjacent hyper-rectangles to make sure we comply to the storage constraint $\mathcal{S}$.

Similarly, we use an indicator $\mathcal{I}(q,p)$ which is 1 when partition $p$ is relevant to query $p$. Taking a SUM(a) query as an example, we define the error introduced by merging partition $p_i, p_j$ as following:
\[
e(p_i, p_j, q) = (1-\mathcal{I}(q, p_i))aggr(a, p_i) + (1-\mathcal{I}(q, p_j))aggr(a, p_j)
\]
And the error for the entire workload:
\[
Error(p_i, p_j, Q) = \sum_{q\in Q}{e(p_i, p_j, q)*w(q)}
\]
Where w(q) is the frequency of query $q$ in the workload if there are duplication for each query.

A bottom up greedy algorithm simply takes the optimal partition as input.

At each iteration it finds and merge the two adjacent partitions of the minimum merging error until the partition size is less than or equal to $\mathcal{S}$.



